The Media Bias Taxonomy: A Systematic Literature Review on the Forms and Automated Detection of Media Bias

The way the media presents events can significantly affect public perception, which in turn can alter people's beliefs and views. Media bias describes a one-sided or polarizing perspective on a topic. This article summarizes the research on computational methods to detect media bias by systematically reviewing 3140 research papers published between 2019 and 2022. To structure our review and support a mutual understanding of bias across research domains, we introduce the Media Bias Taxonomy, which provides a coherent overview of the current state of research on media bias from different perspectives. We show that media bias detection is a highly active research field, in which transformer-based classification approaches have led to significant improvements in recent years. These improvements include higher classification accuracy and the ability to detect more fine-granular types of bias. However, we have identified a lack of interdisciplinarity in existing projects, and a need for more awareness of the various types of media bias to support methodologically thorough performance evaluations of media bias detection systems. Concluding from our analysis, we see the integration of recent machine learning advancements with reliable and diverse bias assessment strategies from other research areas as the most promising area for future research contributions in the field.

==> Chapters/archive/CS_method_old.tex <==
\section{Media Bias Detection Methods} 
%categorization, how and why here?
% Media/Gender Bias in algorithms is left out, mention here or in methods part?

%What is the structure of the different categories? 
%Explain what it is, mention workflow?
%explain what methods were the most common
%mention influential papers and outliers

% Machine Learning - non-transformer-based

% Machine Learning - transformer-based models

% Machine Learning - other ML techniques

% traditional NLP techniques

% graph-based

% datasts
    % granularity of datasets
    % what datasets are they /classification of datasets
    % dataset generation
    % semi-supervised learning, distant supervision, pseudo labelling
%

% Conclusion of the CS methods part?
%
% Outlook: Debiasing / Text neutralization with MLMs like BART (look for discussion in table)




%******************************************
% some stuff that might be reusable from a master thesis
%
%
%************************************************
%************************************************
% Section 3: Existing Approaches
%************************************************
\subsection{Existing Approaches} \label{sec:approaches}
%************************************************
The preceding \autoref{sec:understanding_bias} provides a detailed definition of the concept of media bias. The drawback of the current state-of-the-art research has been outlined, which is the missing of a universal theoretical framework for media bias research. To fill this gap,  the media bias framework has been presented. In addition, media bias has been embedded within the context of other related concepts. Two of these concepts are considered to be particularly important: sentiment analysis and hate speech. As outlined above, hateful language is an indicator of bias. Hence, hate speech detection is relevant when studying media bias. In addition, sentiment analysis is a valuable technique to detect media bias \cite{Enevoldsen_2017, Hamborg_2021, Hube_2018a} and hateful language \cite{Rodriguez_2019}. As a logical implication, sentiment analysis and hate speech detection are relevant related concepts. In the following Section, a brief summary of the current state-of-the-art approaches for the three concepts is provided.
%
%
\hfill \break
%************************************************
% Subsection 1: Media Bias
%************************************************
\subsection{Automated Media Bias Detection} \label{sec:detection_bias}
A glance at the literature reveals that many different approaches for the automatic detection of media bias exist. Roughly, existing work can be split into two areas: those that apply machine learning algorithms to detect bias and those that apply more advanced self-learning models. 

Such machine learning approaches have, for example, been applied by Recasens, et al. \cite{Recasens_2013}, who trained a logistic regression model in order to detect bias-inducing words in a biased sentence. Similar to that, Hube \& Fetahu \cite{Hube_2018a} also trained a supervised model to detect bias on sentence level. A slightly more sophisticated approach has been proposed by Baumer, et al. \cite{Baumer_2015}, who adopt a variety of machine learning algorithms to detect biased language. For example, Stochastic Gradient Descent, Logistic Regression, or k-Nearest Neighbor has been adapted, with the result that Naive Bayes performs best \cite{Baumer_2015}. Testing multiple algorithms and comparing their performance is a common procedure. Spinde, et al. \cite{Spinde_2021a} also have adopted various machine learning approaches to detect bias-inducing words on article level. For example, Linear Discriminant Analysis (LDA), Support Vector Machines (SVM), or Logistic Regression algorithms have been implemented with the result that XGBoost, a decision tree implementation, performs best \cite{Spinde_2021a}. Lastly, another machine learning approach has been proposed by Chen, et al. \cite{Chen_2020b}, who applied a Gaussian Mixture Model to improve bias classification. 

In contrast to that, the use of self-learning language models has become increasingly popular. Applying deep learning approaches like Recurrent Neural Networks (cf. \cite{Hube_2018b, Chen_2020a}) or transformer models like BERT (cf. \cite{Fan_2019, Spinde_2021e}), ELECTRA (cf. \cite{Spinde_2021e}), or XLNet (cf. \cite{Spinde_2021e}) allow for a more advanced classification approach. These neural models enable sequential text processing, which allows capturing the contextual embedding of a word \cite{Hube_2018b} and by that improves bias detection. In addition, the fine-tuning of existing language models with multi-task learning approaches leads to improved media bias detection \cite{Spinde_2022}. Spinde, et al. \cite{Spinde_2022} argue that multi-task learning is especially valuable in cases of scarce data, which applies to media bias detection as high-quality datasets are rare.

Lastly, alternative approaches exist, for example, by Hamborg, et al. \cite{Hamborg_2019} who have pursued an NLP-based approach, where word embeddings have been used to detect bias in news articles.
%
%
\hfill \break
%************************************************
%************************************************
% Subsection 2: Sentiment Analysis 
%************************************************
\subsection{Sentiment Analysis} \label{sec:sentiment_analysis}
Studying the literature for sentiment analysis reveals that the number of existing approaches can be divided into three main areas. First, the most basic approaches for sentiment analysis are lexical approaches. The main idea is to create word lexicons that contain for each word its polarity (positive, negative) \cite{Bhadane_2015, Drus_2019}. In the literature, some of these dictionaries are referenced. First, there are dictionaries like LIWC\footnote{https://www.liwc.app/}, Harvard's General Inquirer (GI)\footnote{http://www.mariapinto.es/ciberabstracts/Articulos/Inquirer.htm}, or Cambridge's Hu-Liu04\footnote{https://www.cs.uic.edu/~liub/FBS/sentiment-analysis.html} lexicon, which contain a binary label for each word's polarity (positive, negative) \cite{Hutto_2014}. However, other dictionaries exist where words are linked to sentiment intensity, for example, SentiWordNet or SenticNet \cite{Hutto_2014}. Given such lexicons, the overall polarity of a sentence can then be determined by adding up each word's polarity \cite{Bhadane_2015}. For example, Enevoldsen \& Hansen \cite{Enevoldsen_2017} applied such a dictionary-based approach to detect the sentiment of Danish newspaper articles. The authors derived the mean sentiment score for each article based on the Danish sentiment dictionary AFINN \cite{Enevoldsen_2017, Nielsen_2011}. Just recently, Dubey \cite{Dubey_2020} adapted a lexical approach to classify Twitter data on COVID-19 with regard to sentiment. The author used the R package "syuzhet"\footnote{https://cran.r-project.org/web/packages/syuzhet/vignettes/syuzhet-vignette.html}, which "classifies the tweets on the basis of sentiments (positive and negative) and also categorizes them into 8 emotions" \cite[3]{Dubey_2020}. 

Another large area of sentiment analysis research focuses on the application of machine learning approaches to detect bias. Common algorithms like Naive Bayes, Support Vector Machines, Ensemble Learner, or Maximum Entropy have been used to detect a statement's sentiment (cf. \cite{Neethu_2013, Go_2009, Hemalatha_2013}). The existing literature shows that the most frequently used algorithms for sentiment detection are Support Vector Machines and Naive Bayes \cite{Bhadane_2015}. Some scholars also propose combined approaches \cite{Drus_2019}, for example, Joyce \& Deng \cite{Joyce_2017} using the OpinionFinder Lexicon \cite{Wilson_2005} together with Naive Bayes algorithm to get the sentiment of tweets. 

Similar to media bias detection, an increasing amount of researchers implement more advanced deep learning approaches to detect sentiment. For example, Wang, et al. \cite{Wang_2016} have proposed a CNN-LSTM model that is able to differentiate partial information from the text input. Other neural network-based approaches consider variations of Recurrent Neural Networks (cf. \cite{Agarwal_2019}) or applied combined attention-based approaches (cf. \cite{Basiri_2021}). In order to overcome shortcomings of, for example, Recurrent Neural Networks, Transformer based architectures are proposed (cf. \cite{Jiang_2019, Gao_2019}). 
%
%
\hfill \break
%************************************************
%************************************************
% Subsection 3: Hate Speech 
%************************************************
\subsection{Automated Hate Speech Detection} \label{sec:detecting_hate}
Given the large amounts of hate speech research, existing work can be divided into three categories. The first category refers to rule-based approaches \cite{Mohiyaddeen_2021, Alrehili_2019}. The idea behind these methods is that the text is classified for hate based on a set of rules. These rules are manually created but enriched by word lists and linguistic cues, for example, grammar, morphology, or semantics \cite{Mohiyaddeen_2021, Alrehili_2019}. For instance, Gitari, et al. \cite{Gitari_2015} build a rule-based classifier to detect hate speech, using three features: word polarity, a hate lexicon, and grammatical patterns \cite{Gitari_2015}. Such rule-based approaches usually achieve high accuracy but are very time-intense \cite{Alrehili_2019}. Rodríguez, et al. \cite{Rodriguez_2019} introduce a different approach whose goal is to detect hate speech on Facebook. To achieve this, the authors first deduce a sentiment analysis and then clustered the posts accordingly \cite{Rodriguez_2019}. 

Another part of existing research applies machine learning algorithms to build a hate speech classifier \cite{Mohiyaddeen_2021}. Similar to media bias detection and sentiment analysis, standard algorithms are used, for example, Support Vector Machines (cf. \cite{Smedt_2018, Warner_2012}) or Logistic Regression (cf. \cite{Davidson_2017}). In addition, existing literature proposes that hate speech is a multi-class classification problem rather than binary class. For example, Davidson, et al. \cite{Davidson_2017} point out that supervised machine learning methods are error-prone as they fail to detect the slight differences between hateful language and other kinds of offensive language. 

The third category of automated hate speech detection refers to deep learning approaches \cite{Mohiyaddeen_2021}. The state-of-the-art approaches for hate speech detection are similar as already mentioned for media bias detection and sentiment analysis. For example, approaches exist where variations of Convolutional Neural Networks are implemented (cf. \cite{Zhang_2018a, Zhang_2018b}) or where multi-task learning approaches are combined with a BERT-based language model \cite{Mozafari_2020}.
%
%
\hfill \break
%************************************************
%************************************************
% Subsection 4: Summary Approaches 
%************************************************
\subsection{Summary: State-of-the-Art Approaches} \label{sec:summary_approaches}
What has been outlined in this \autoref{sec:approaches} is that similar state-of-the-art approaches for all three concepts exist. This is no surprise as media bias detection, sentiment analysis, and hate speech detection are all three a subtask of text classification. From a broader perspective, supervised machine learning and deep neural models are promising approaches for the three concepts. In general, the implementation of transformer language models has a wide range of applications, where media bias detection, sentiment analysis, and hate speech detection are only a small variety. In most cases, these more sophisticated models outperform the supervised learning approaches.
%
%

\hfill \break
%************************************************
%************************************************
% Section 4: Datasets
%************************************************
\section{Existing Datasets} \label{sec:datasets}
As demonstrated in \autoref{sec:approaches} a large variety of different text classification approaches exists. These techniques usually require labeled data for the training or fine-tuning process of the particular algorithm. However, collecting sufficient amounts of data and getting high-quality annotations is difficult \cite{MacAvaney_2019, Spinde_2022}. In the following, a listing of existing datasets for media bias detection, sentiment analysis, and hate speech detection is provided.
%
%
\hfill \break
%************************************************
%************************************************
% Subsection 1: Media Bias
%************************************************
\subsection{Media Bias Datasets} \label{sec:datasets_bias}
For media bias research, most of the existing datasets provide annotations on sentence level \cite{Recasens_2013, Hube_2018b, Hube_2018a, Färber_2020, Lim_2020, Chen_2020a} with some having additional information on word-level \cite{Baumer_2015, Spinde_2021f, Spinde_2021e}, but a few exceptions provide labels on article-level \cite{Lim_2018b, Cremisini_2019, Fan_2019}. A few of the articles are domain-specific, i.e., referring to only one news event or topic \cite{Baumer_2015, Lim_2018b, Cremisini_2019, Färber_2020}, but most of the data refers to several topics. In the following, an overview is provided.
%
\begin{itemize}
    \item \emph{\textbf{NPOV Corpus - 1 \cite{Recasens_2013}.}} NPOV stands for "neutral point of view" and refers to Wikipedia's policy to ensure that all articles are written from a fair and non-biased point of view\footnote{https://en.wikipedia.org/wiki/Wikipedia:Neutral\_point\_of\_view}. Recasens, et al. \cite{Recasens_2013} created a dataset by extracting all articles that had been in Wikipedia's category of NPOV disputes\footnote{https://en.wikipedia.org/wiki/Category:All\_Wikipedia\_neutral\_point\_of\_view\_disputes} and then further split the articles into sentences. Each article consists of a set of revisions, i.e., different versions of the article. The authors then extracted all words that had been changed from one version to the other, called edits. Hence, each edit contains of a before word and an after word. 
    \item \emph{\textbf{NPOV Corpus - 2 \cite{Hube_2018b}.}} Hube \& Fetahu \cite{Hube_2018b} also created a dataset by collecting all Wikipedia articles that had been in Wikipedia's category of NPOV. The authors then asked crowdsource workers to annotate each statement with regard to the presence of bias. The final dataset contains statements labeled as biased or neutral.  
    \item \emph{\textbf{Wikipedia dataset \cite{Hube_2018a}.}} Hube \& Fetahu \cite{Hube_2018a} created a dataset by collecting the latest Wikipedia articles with each statement being labeled as biased or unbiased. 
    \item \emph{\textbf{Framing dataset \cite{Baumer_2015}.}} Baumer, et al. \cite{Baumer_2015} published a domain-specific dataset by collecting political news articles. The final dataset consists of a number of articles where each word has been annotated for framing.
    \item \emph{\textbf{Single-event articles \cite{Lim_2018b}.}} This dataset created by Lim, et al \cite{Lim_2018b} contains news articles to one single event, "Black men arrested in Starbucks", that has been annotated with the labels not biased, slightly biased, fairly biased, and strongly biased.
    \item \emph{\textbf{Ukraine crisis dataset - 1 \cite{Cremisini_2019}.}} Cremisini, et al. \cite{Cremisini_2019} present a dataset that contains news articles that are related to the Ukraine crisis. Each article was manually rated as either pro-Russian, pro-Western, or neutral.
    \item \emph{\textbf{Ukraine crisis dataset - 2 \cite{Färber_2020}.}} Färber, et al. \cite{Färber_2020} extended the previously mentioned dataset by Cremisini, et al. \cite{Cremisini_2019} by annotating it on sentence-level with regard to bias dimensions. These dimensions are Hidden Assumptions and Premises, Subjectivity Framing, and Overall Bias.
    \item \emph{\textbf{MBIC \cite{Spinde_2021f}.}} MBIC stands for Media Bias Including Characteristics and is a dataset compiled by Spinde, et al. \cite{Spinde_2021f}. This dataset consists of sentences that had been annotated for bias with labels on sentence-level and word-level. On sentence-level, annotators had been asked to label the sentence as biased or non-biased and if the sentence expresses an opinion. On word-level, annotators had to state which the bias-inducing words are. 
    \item \emph{\textbf{BABE \cite{Spinde_2021e}.}} BABE stands for Bias Annotations By Experts and is a dataset that was built on top of MBIC \cite{Spinde_2021e, Spinde_2021f}. It contains sentences that have been labeled on sentence-level and word-level by expert annotators. The annotator-schema was the same as for MBIC \cite{Spinde_2021e}.
    \item \emph{\textbf{BASIL \cite{Fan_2019}.}} BASIL stands for Bias Annotation Spans on the Informational Level and is a dataset created by Fan, et al. \cite{Fan_2019}. The authors collected sets of articles where each set refers to a similar news event. The articles have been annotated on the article level with labels on the overall polarity and on sentence-level with labels on bias type, bias target, bias polarity, bias aim, and whether the biased statement is a quote.
    \item \emph{\textbf{LimA \cite{Lim_2020}.}} This dataset, conceived by Lim, et al. \cite{Lim_2020} consists of sentences referring to four different events. The sentences had been annotated by crowdsource workers with labels on the sentence's bias.
    \item \emph{\textbf{ChenA \cite{Chen_2020a}.}} Chen, et al. \cite{Chen_2020a} created this dataset by first collecting articles from \emph{allsides.com\footnote{https://www.allsides.com/unbiased-balanced-news}}, containing labels on topic and political bias. Then the authors added a fairness label provided by ad fontes media. Lastly, each sentence had been labeled either as political bias, unfairness, or non-objectivity, where the labels were in turn derived from the ad fontes media labels.  \\
\end{itemize}
%
%************************************************
%************************************************
% Subsection 2: Sentiment Analysis
%************************************************
\subsection{Sentiment Analysis Datasets} \label{sec:datasets_sentiment}
The majority of existing sentiment datasets are compiled of Twitter data \cite{Go_2009, Saif_2013, Thelwall_2011, SemEval}, only the dataset created by Hamborg \& Donnay refers to newspaper articles \cite{Hamborg_2021}. However, the annotation schema varies between the different datasets. Some contain sentiment labels on tweet-level \cite{Go_2009, Thelwall_2011, SemEval}, whereas others sentiment information on target-level \cite{Hamborg_2021, Saif_2013}. Also, the terms used to label sentiment and the number of sentiment classes are inconsistent. The most general case is labels for positive, negative, and neutral \cite{Go_2009, Thelwall_2011}, but sometimes sentiment classes are added, for example, a label for mixed sentiment or other \cite{Saif_2013}.
%
\begin{itemize}
    \item \emph{\textbf{Stanford Twitter Sentiment (STS)\footnote{http://help.sentiment140.com/home} \cite{Go_2009}.}} This sentiment dataset has been compiled by Go, et al. \cite{Go_2009} and contains tweets labeled as positive, negative, or neutral. It consists of a training set and a test set, with the test set being manually labeled. 
    \item \emph{\textbf{STS-Gold \cite{Saif_2013}.}} This corpus has been constructed based on the STS dataset, but annotations are on tweet and target level. The number of labels have been expanded by adding the two additional labels mixed, and other \cite{Saif_2013}.
    \item \emph{\textbf{Sentiment Strength Twitter dataset (SS-Twitter)\footnote{http://sentistrength.wlv.ac.uk/documentation/} \cite{Thelwall_2011}.}} This dataset has been constructed by Thewall, et al. \cite{Thelwall_2011} and contains tweets that have been annotated for their sentiment strength. This means, labels for negative sentiment are on a scale from -1 (not negative) to -5 (extremely negative), and on a scale from 1 t0 5 for positive sentiment respectively \cite{Thelwall_2011}.
    \item \emph{\textbf{SemEval  datasets\footnote{https://semeval.github.io/} \cite{SemEval}}} SemEval is a once-a-year international workshop on semantic evaluation. As part of the event, the respective datasets are provided for download. For example, the SemEval2014 dataset\footnote{https://alt.qcri.org/semeval2014/task9/index.php?idDdata-and-tools} contains Twitter data which have been labeled on tweet-level as positive, negative, or neutral \cite{Jianqiang_2017}. Datasets from other years exist as well \cite{Saif_2013}.
    \item \emph{\textbf{NewsMTSC\footnote{https://github.com/fhamborg/NewsMTSC} \cite{Hamborg_2021}.}} This dataset created by Hamborg \& Donnay \cite{Hamborg_2021} contains sentences that were annotated with labels on the sentence's target and whether the polarity towards the target is positive, negative, or neutral.\\
\end{itemize}
%
%
%************************************************
%************************************************
% Subsection 3: Hate Speech
%************************************************
\subsection{Hate Speech Datasets} \label{sec:datasets_hate}
The vast majority of hate speech datasets consist of social media data like Twitter \cite{Davidson_2017, Waseem_2016b, Waseem_2016a} or Stormfront \cite{deGibert_2018}, a white supremacist forum. Some of the data have binary labels \cite{deGibert_2018}, although the majority of annotations consist of three or four labels \cite{Davidson_2017, Waseem_2016b, Waseem_2016a, SemEval, Kaggle}. To ensure transparency, the names for the datasets in the following list have been adopted from MacAvaney, et al. \cite{MacAvaney_2019}.
%
\begin{itemize}
    \item \emph{\textbf{HatebaseTwitter\footnote{https://github.com/t-davidson/hate-speech-and-offensive-language} \cite{Davidson_2017}.}} This dataset has been created by Davidson, et al. \cite{Davidson_2017} and consists of Twitter data. The tweets have been labeled as hate speech, offensive language, or neither.
    \item \emph{\textbf{WaseemA\footnote{http://github.com/zeerakw/hatespeech} \cite{Waseem_2016b}.}} This dataset also contains of Twitter data and was annotated with labels for racist, sexist, or neither.
    \item \emph{\textbf{WaseemB\footnote{http://github.com/zeerakw/hatespeech} \cite{Waseem_2016a}.}} With this dataset, Waseem \cite{Waseem_2016a} extended the previously created dataset by Waseem \& Hovy \cite{Waseem_2016b}. The annotation schema is similar to WaseemA, except that one more label has been added. Hence, this dataset categorizes Twitter data into racist, sexist, neither, or both. 
    \item \emph{\textbf{Stormfront\footnote{https://github.com/Vicomtech/hate-speech-dataset} \cite{deGibert_2018}.}} This dataset contains binary annotated data from Stormfront. The labels are either hate or no hate. 
    \item \emph{\textbf{HatEval\footnote{https://competitions.codalab.org/competitions/19935} \cite{SemEval}.}} This dataset is from the SemEval competition 2019 (Task 5) and is annotated on hate and aggression, and additionally contains a label for the sentence's target \cite{MacAvaney_2019, SemEval}.
    \item \emph{\textbf{Kaggle\footnote{https://www.kaggle.com/c/detecting-insults-in-social-commentary} \cite{Kaggle, MacAvaney_2019}.}} This dataset was published by Kaggle for one of Kaggle's competitions. The data used for this competition is social media data and contains binary labels on insult \cite{MacAvaney_2019, Kaggle}. \\
\end{itemize}
%
%
%************************************************
%************************************************
% Subsection 3: Summary
%************************************************
\subsection{Summary: Existing Datasets} \label{sec:summary_datasets}
In sum, a wide range of datasets for the three tasks exists but with the drawback that annotations are not uniform. The respective labels are often against the background of various media bias types for media bias. For example, the dataset of Baumer, et al. \cite{Baumer_2015} refers to framing bias, whereas the dataset of Chen, et al. \cite{Chen_2020a} aims to detect more detailed types of media bias. Some researchers even completely adjust the dataset labels to match their respective research goals, for example, by labeling sentences as pro-Russian, pro-Western, or neutral \cite{Cremisini_2019}. A similar problem occurs for sentiment datasets, as some datasets label the sentiment polarity (cf. \cite{Go_2009, SemEval}), whereas others measure the strength of the polarity (cf. \cite{Thelwall_2011}). Unsurprisingly, the same ambiguity occurs for hate speech datasets, as some data are labeled for hate, others for insult or aggression.

Also, the label target is not always comparable, as in some datasets the labels are on statement-level (cf. \cite{Recasens_2013, Go_2009, Davidson_2017}), for others its on article-level (cf. \cite{Lim_2018b, }), and in some cases the annotations are even target-related (cf. \cite{Hamborg_2021}).

% Some sources that were formerly in the linguistic section. Inspect and delete if irrelevant, otherwise add were suitable.

%Hatespeech due to linguistic media bias is difficult to find ---- done one

%https://www.sciencedirect.com/science/article/pii/S0306457321000157 --- done

%https://www.degruyter.com/document/doi/10.1515/opli-2020-0028/html --done

%https://journals.sagepub.com/doi/abs/10.1177/0261927X16666884 --done

%http://www.journals.aiac.org.au/index.php/IJALEL/article/view/5984 --done

%https://mediabiasanal-iwf8969.slack.com/files/U01T18NPDRA/F021UD26R4M/webson_et_al._2020_-_are_illegal_aliens_the_same_as_undocumented_workers.pdf

%https://mediabiasanal-iwf8969.slack.com/files/U01T18NPDRA/F022A410AGZ/chakrabarty_et_al._2021_-_entrust.pdf

%https://mediabiasanal-iwf8969.slack.com/files/U01T18NPDRA/F022M9JG6JC/rashkin_et_al._2016_-_connotation_frames._a_data_driven_investigation_.pdf

%https://mediabiasanal-iwf8969.slack.com/files/U01T18NPDRA/F021UD26R4M/webson_et_al._2020_-_are_illegal_aliens_the_same_as_undocumented_workers.pdf

\subsection{Preprocessing}
\subsection{Detection of Gender Bias}
\subsection{Detection of Racial Bias}
%Copied from Social Science, inspect, otherwise delete
Recently, research works are also conducted to analyse media portrayals that can sometimes trigger racial stereotypes and portray the victims detrimentally. In \citep{articleduke}, the authors have carried out an experiment to perform a quantitative analysis on the effects of racially biased media reports with the perception of victim-blaming and justification of the lethal action. Through their experiment conducted to identify media bias, they argue that negative stereotypical information reported by media can cause victim-blaming and criticize the victim for their own death/harm. Similarly, there are also study conducted on gender bias from a social scientific perspective. 
%Copied from Social Science, inspect, otherwise delete
Studies are also conducted to reveal the influence of media on promoting racial bias.
One such works include \citep{10.1111/j.1460-2466.2012.01672.x}, where the author focused on the effects of media on immigrants. He executed content analysis on the campaign held for the naturalization of immigrants in Switzerland. The analysis was carried out on 947 articles from the German and French-speaking parts of the country containing arguments demonstrated by the politicians or journalists. The survey method was conducted as a two-wave panel survey through telephone interviews with a gap of one month between the two interviews. During the gap, the  participants had the probability of watching either a positive news portrayal or a negative news portrayal of the immigrants. Based on these data received from the survey and through content analysis, the authors inspected the attitudes towards the campaign. The study revealed that exposure to negative news about immigrants promoted a negative attitude towards the immigrants.
A similar approach, based on content analysis was carried out in \citep{pub.1002980197}. The authors assessed the racial bias present in the local television news in Los Angeles and Orange counties in the U.S. Their findings revealed that the minority group including Blacks and Latinos are promoted as lawbreakers in a more likely manner than the Whites.
\subsection{Detection of Framing Effects}
%Copied from former Linguistics, inspect, otherwise delete
\citep{10.1145/3204948} recognizes framing bias present in the sentences of the news articles referring to the subject of ``the construction of a ballistic missile defense system in Europe". The features obtained using linguistic analysis of the text content and language patterns are utilized in identifying the frame in the sentence by developing different machine learning classifiers to automatically identify the bias at various levels of granularity. They identify the bias using linguistic indicators such as``type and polarity of frame in a sentence". This paper serves as an example of the interdisciplinary approach of including linguistic science and computer science in detecting framing bias in the media. 
%check
In a similar approach of combining linguistic analysis with machine learning, \citep{8215582} analysed the quotation patterns and the word choices including direct and indirect speech used by the political parties as reported in two news articles from UK. They examined political speeches present in articles the \emph{Guardian} and the \emph{Telegraph} and used a Random Forest classifier to identify the selection, coverage and framing bias present in the speech through exploring, the unique linguistic presentation of the same events in two different news outlets.
\subsection{Detection of Bias By Word Choice}
\subsection{Detection of Related Concepts}
\subsection{Evaluation of Classifiers / Conclusion }

\section{Computer Science Research on media bias} 
% left fixed width:
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
 
% center fixed width:
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
 
% flush right fixed width:
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}
\begin{table}[]
\begin{tabular}{L{2cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|l}

 & 2019 & 2020 & 2021 & 2022 & total \\\hline
other ML techniques & \cite{ anthonio_team_2019, dinkov_predicting_2019, baly_multi-task_2019, sapiro-gheiler_examining_2019} & \cite{ leavy_uncovering_2020, bourgeois_selection_2018, stefanov_predicting_2020, mokhberian_moral_2020, alzhrani_ideology_2020, kameswari_enhancing_2020, ganguly_empirical_2020, chen_detecting_2020, shahid_detecting_2020, van_den_berg_context_2020, hamborg_bias-aware_2020} & \cite{ orbach_out_2020, spinde_mbic_2021, cuellar-hidalgo_luc_2021, zhou_hidden_2021, rao_gender_2021, spinde_automated_2021, bauer_analyzing_2021, krommyda_experimental_2021} &  & 23 \\\hline
non-transformer-based & \cite{ han_fallacy_2019, hube_neural_2019, bordia_identifying_2019, ananya_genderquant_2019, gangula_detecting_2019} & \cite{ baly_we_2020, field_unsupervised_2020, xiao_timme_2020, cruz_document_2020, hube_methods_2020, mathew_hatexplain_2020, lazaridou_discovering_2020, jiang_comparing_2020, webson_undocumented_2020, chen_analyzing_2020} & \cite{ ruan_pseudo-labelling_2021, sinno_political_2022, hamborg_newsmtsc_2021, cuellar-hidalgo_luc_2021, gerald_ki_wei_huang_hyperpartisan_2021, ruan_bias_2021, spinde_automated_2021, krommyda_experimental_2021} & \cite{ liu_political_2021, fagni_fine-grained_2022} & 25 \\\hline
traditional NLP techniques & \cite{ wevers_using_2019, badjatiya_stereotypical_2019, taylor_illegal_2019, sapiro-gheiler_examining_2019, cornelissen_computational_2019} & \cite{ leavy_uncovering_2020, zahid_modeling_2020, niven_measuring_2020, ferrer_discovering_2020, papakyriakopoulos_bias_2020, de_arruda_analysing_2020, aires_information_2020, mendelsohn_framework_2020} & \cite{ koprinska_media_2020, dalonzo_machine-learning_2021, toeppe_identification_2021, kroon_guilty_2021, Kwak_2021, dacon_does_2021, sales_assessing_2021} &  & 20 \\\hline
transformer-based & \cite{ han_fallacy_2019, gao_target-dependent_2019, dinkov_predicting_2019, fan_plain_2019, pryzant_automatically_2019} & \cite{ baly_what_2020, baly_we_2020, li_using_2021, pant_towards_2020, nadeem_stereoset_2021, stefanov_predicting_2020, PoliBert20, hamborg_newsalyze_2020, mokhberian_moral_2020, vig_investigating_2020, bhardwaj_investigating_2021, tran_how_2020, mathew_hatexplain_2020, mozafari_hate_2020, chen_detecting_2020, van_den_berg_context_2020, jiang_comparing_2020, kwak_systematic_2020} & \cite{ huguet_cabot_us_2021, blackledge_transforming_2021, kameswari_towards_2021, madanagopal_towards_2021, ruan_pseudo-labelling_2021, sinno_political_2022, orbach_out_2020, hamborg_newsmtsc_2021, hamborg_newsalyze_2021, spinde_neural_2021, hofmann_modeling_2021, zhou_hidden_2021, sinha_determining_2021, he_detect_2021, ruan_bias_2021, bauer_analyzing_2021, spinde_interdisciplinary_2021, liu_transformer-based_2021} & \cite{liu_politics_2022, lee_neus_2022, spinde_exploiting_2022, raza_dbias_2022, krieger_2022} & 8 \\\hline
graph-based &  & \cite{ stefanov_predicting_2020, chen_neutral_2021, chitra_analyzing_2020} & \cite{ zhou_uncovering_2021, hofmann_modeling_2021, villa_echo_2021, guimaraes_characterizing_2021} & \cite{ guo_modeling_2022} &  \\\hline
total & 17 & 41 & 34 & 46 & 8
\end{tabular}
\end{table}
In this section, we analyze how different approaches and aspects considered in various research works from the field of computer science contribute in studying media bias. In order to detect the bias effectively, recent advancements in automated methods of computer science aid in extracting beneficial information from unstructured data that include text and speech \citep{MONTOYO2012675}. %2012
Devising mechanisms to analyze and identify bias such as information bias in textual content helps in delivering unbiased information to the readers  \citep{inproceedings_B}. %2018
%`` quality and fairness of the information delivered to the citizens". 
The news content leading to such kind of bias often includes sentences or clauses that convey information which is conjectural to the main event covered throughout the article \cite{chen2020detecting}. This article level bias detection is handled successfully by taking leverage of second-order sentence-level features such as probability distributions of the frequency, positions, and sequential order of lexical and informational sentence-level bias utilizing a Gaussian Mixture Model \cite{chen2020detecting}.
\newline
Another concept pertaining to media bias is event selection, which determine the factors responsible for the event coverage by the news sources based on the physical location along with the timeline\citep{10.1086/316964}.
%``how the news media cover events in all times and all places" 
In an attempt to analyze such kind of bias, \citep{sholar2016predicting} explored the patterns of news coverage and their corresponding headlines in various news articles concerning the events related to Israel in 2014. By employing Multiclass Naive Bayes and SVM models to classify the news source that published a given article based on the headlines of the article, the authors revealed the correlation between each news source's political leanings and the keywords used in the headlines to be significant.

News coverage and media's contribution in reporting events that include race/ethnicity have a strong impact on the public. Media fails to cover the racial minorities in the way that the majorities within that society are covered \citep{doi:10.1177/107769909206900110}. 
%2012
In a recently published study \citep{doi:10.1177/1077699020932304} %2021
, the authors have analyzed over 3 million Dutch news articles on an account of investigating any form of stereotypical content referring the ethnic minorities and then to identify the ethnic bias present in the news content. They used word embeddings in detecting the implicit bias present in news coverage. The authors argue that few other automated approaches on detecting ethnic bias primarily rely on the approaches dealing with bag-of word approaches \citep{10.1080/15205436.2018.1442479, doi:10.1177/1081180X06297436} %2018, 2007
where co-occurrences of words such as Muslims and terrorists are analyzed rather than the contextual information such as in word embeddings. In contrast to this, there are studies \citep{GargE3635, sweeney-najafian-2019-transparent} which claim that word embeddings are trained using corpora containing bias in them hence, these word embeddings reflect their bias in the language models using the embeddings and in turn are biased. Considering the complications involved in identifying media bias and its causes, new tools and automated methods are developed that assist in assessing the bias and also in identifying the genuineness of the content \citep{abs-1904-01531}.
The content of media communication and reports can portray gender hierarchy and promote gender inequalities hence, there is a need for humans and algorithms in curating the gender biased content \citep{doi.org/10.1002/asi.24335}.  In a recent study \citep{Asr2021}, a software system ``Gender Gap Tracker" was developed, that analyzes syntactic structure of sentences of the news content and utilizes Named Entity recognition to predict the gender in order to, identify the proportion of females and males represented in news articles. The tool is devised to address and assess the gender parity that exists in media outlets and sources.
\newline
Similarly, in an attempt to identify the significance of news articles posted in news websites, that can potentially lead to hateful activity in the comments section of the articles, a quantitative analysis of news content was carried out by the authors of \citep{10.1145/3394231.3397902}. A content analysis was performed on the articles using a text analysis tool ``LIWC" and a hatespeech classifier ``Perspective API"  which can handle swear words robustly to identify the abusive comments. Upon analysis, the authors concluded that, news articles influencing more hateful comments contain different linguistic pattern than the other articles.
%%Until Here%%%%%
%A study \cite{chen2020detecting} that focuses on identifying media bias by analysing sentence-level and article-level features in an existing media bias dataset by utilizing a Gaussian Mixture Model. The authors explored the effectiveness of using secondary information such as probability distributions of the frequency, positions, and sequential order of lexical and informational sentence-level bias in the model and successfully tackled article-level bias detection.



%has started gaining attention only recently. 

%There have been quite some researches done focusing on machine learning models to automatically identify media bias.
 
%One such methods is presented in \cite{chen2020detecting} where, the authors study the effectiveness of utilizing secondary information such as probability distributions of the frequency, positions, and sequential order of lexical and informational sentence-level bias in a Gaussian Mixture Model in identifying the bias.

%about biased statements in an article helps to improve detection effectiveness the Gaussian Mixture Model performs when, including sentence-level bias features in bias detection can affect the political bias of the whole article and outperform other models which do not include the sentence-level information. They use a dataset that includes manually annotated bias labels at article level as well as lexical and informational bias labels at sentence level to train their model. In order to investigate the sentence-level bias they analyze the bias features such as frequency and position of the biased statements and also the bias sequence. To extract the features they use different machine learning models such as SVM, Naive Bayes and a first order Markov Model.


%In a survey by \citep{app11073184}, different machine learning models are explored that detect and mitigate bias including media bias. 

%An approach based on news article similarity is devised in \citep{inproceedings_B} using various machine learning approaches such as Naive bayes, Logistic regression and SVM (Support Vector Machine) in Polish news articles. The author develops these systems to automatically identify the articles that present same news/events and then to analyse them comparatively to detect bias. They also provide another approach where, they predict the news source based on it's content and when predicted correctly the source is mostly considered to be biased.
%2018!!!!


%When dealing with different types of bias, event selection plays a significant role in the creation of biased news coverage. In \citep{sholar2016predicting} the authors focus on dealing with event selection bias in different news sources. They used classifiers such as SVM, Naive bayes and trained them to map headline keywords with the respective news sources. The study found a significant correlation between the keywords mapped with the respective news sources and the political inclination of each news outlet.  

%the authors used a topic-modelling approach which is a combination of LDA (Latent Dirichlet Allocation) and different NLP methods. They extracted topics from some of the politically inclined U.S. news magazines to form a corpus and then analyzed the news coverage and media bias in a better way using their model. There are various studies(....) basing their findings on the 'right' data to be used to mitigate bias in the models developed for various technological applications.


%\hl{In the area of NLP, word embeddings and language models are widely used. These models often are trained using large sets of data acquired from different sources, there is a possibility that these data may contain stereotyped biased knowledge and generate biased language models hence, the authors of} \citep{garrido2021survey}  \hl{argue that 'fairness' to be considered when developing such models.}

%TODO Smi here

%However in contrast to these approaches, a literature survey \citep{blodgett2020language}\hl{ conducted on 146 papers analyzing 'bias' in general including media bias have argued that "their motivations are often vague, inconsistent, and lacking in normative reasoning; and their proposed quantitative techniques for measuring or mitigating 'bias' are poorly matched to their motivations and do not engage with the relevant literature outside of NLP". They suggest that relationships between language, social hierarchies and NLP techniques is a step forward to better understand the concept of bias and thereby identifying and mitigating the bias in a better way.} 

%https://www.aclweb.org/anthology/2020.lrec-1.159.pdf

%https://www.aclweb.org/anthology/2020.acl-main.106/

%https://www.aclweb.org/anthology/2020.socialnlp-1.1.pdf  -- wip (jerome)
\citet{kameswari-etal-2020-enhancing} show a correlation between presuppositions and bias in news articles. They present a dataset consisting of 200 unbiased and 850 biased articles written in Telugu, a low resource language. Additionally to bias labels on the article-level, sentences containing presuppositions, i.e. information the reader is not expected to know, are labeled accordingly. The authors train multiple simple classifiers, using NB, SVMs, Multi Layer Perceptrons (MLP) and others. To show that detecting political bias can be facilitated using knowledge about presuppositions in the text, \citet{kameswari-etal-2020-enhancing} conduct experiments with and without their additional features and report improvements of around 5 to 20 percentage points in accuracy for each of the classifiers.  
This indicates that incorporating knowledge of presuppositions in a classifier can generally improve its performance. However, the authors conduct their experiments on a newly introduced dataset which complicates comparisons. Furthermore, they conduct their experiments using simple methods only and don’t examine the influence on state-of-the-art attention-based neural models. 

%https://www.sciencedirect.com/science/article/pii/S0306457321000157  
As mentioned earlier, apart from media platforms, search engines, online digital platforms and social media also often serve as gatekeepers for various kinds of information \citep{bhargava2002paid}.






%to  journalists in identifying the gender gap and present news events pertaining to more diversified gender voices. They have developed a software named 'Gender Gap Tracker' which basically is a NLP technology based system that uses big storage of data containing news stories collected on a daily basis from Canadian media and seven English news sites. The tracker displays the ratio of different genders and raw numbers mentioned in the respective news stories along with a bar chart for each news source. The tracker works by processing the collected data and then predicting the gender using NER (Named Entity Recognition) and gender predicting web services. They suppose that, the software creates awareness on gender parity amongst the media and news sources and aids in reducing the gap.


%https://journals.plos.org/plosone/article?id=10.1371/journal.pone.0245533

%sudha

%https://arxiv.org/pdf/2005.12246




%The research conducted by \citep{10.1145/3394231.3397902}, analyze the online news sources and present what kind of news articles attract hateful/abusive comments and methods to identify them. The authors investigate 412K news articles of UK and U.S. origin which are both biased and unbiased containing 125M users comments on the whole. To identify the biased nature of the articles they use the information from Media Bias/Fact Check (MBFC)(.....) website. To identify hate speech in the collected data they use the Logistic Regression based classifier 'Hatesonar'(..) and 'Perspective API' (...) which uses different machine learning models to identify toxic/hateful/abusive present in the text.They provide a conclusion depending on their analysis that, the news sites which are biased contain more hateful comments that the unbiased sites. However, there are few limitations in the approach such as, depending on third party machine learning API to detect the hate speech and detecting all types of hate speech is not possible.

\subsection{Methods to identify other related concepts}
We will now briefly touch on methods to detect other phenomena that occur in the media landscape and which are closely related to the concept of media bias. Additionally, we will  discuss some methods that may be used and combined to improve the result in media bias detection or that could serve as a starting point to develop new approaches. Finally, we will present neutralization as a relatively new task in the domain of media bias mitigation.

Even though fake news and rumors are both conceptually distinct from media bias, they too distort the perception of reality and hence have similar societal consequences. This shared effect relates the three concepts to each other conceptually. 
It is furthermore reasonable to assume that fake and biased news disseminate similarly which makes it all the more attractive to investigate propagation-based and content-independent methods in related areas.
% TODO: Maybe add definition of fake news and rumor
% FAKE NEWS DETECTION
% 02_orc https://arxiv.org/abs/2007.03316
\citet{DBLP:journals/corr/abs-2007-03316} try to identify fake news in social media (Twitter) using propagation-based techniques, i.e. the way how fake news spread, without relying on textual information about the content. 
They argue that this is particularly useful as propagation-based approaches are both, less vulnerable to adversarial attacks and language agnostic. 
Based on the FakeNewsNet dataset \citep{DBLP:journals/corr/abs-1809-01286}, the authors create graphs for each item of news where each node refers to a user/ tweet. 
A user is represented using only non-textual features like number of friends and followers, verification status and others. Additionally, they model user interaction in a separate, weighted graph and train graph neural networks (GNN)s on both graphs alone as well as on a combination of both feature sets. 
\citeauthor{DBLP:journals/corr/abs-2007-03316} also propose a technique to ensure that the models perform well on new, potentially entirely different graphs and report that their models achieve comparable or superior performance to state-of-the-art methods like dEFEND \citep{10.1145/3292500.3330935} and CSI \citep{10.1145/3132847.3132877} by only using non-textual features. 
% FAKE NEWS DETECTION
% 03_orc https://www.aclweb.org/anthology/2020.acl-main.48.pdf 
Similarly, \citeauthor{lu-li-2020-gcan}'s \citep{lu-li-2020-gcan} model GCAN (Graph-aware Co-Attention Network) also primarily focuses on the sequence of retweets. In addition, GCAN takes into account the short text content of the source tweet and features extracted from the user profiles. The authors further add a graph-aware propagation representation using a graph convolutional network (GCN) to model the interactions among users who are involved in the cascading of the same source tweet. In their work, \citeauthor{lu-li-2020-gcan} propose a dual co-attention mechanism that aligns the source tweet with user propagation embeddings and graph-aware interaction embeddings respectively. Intuitively, this conveys information about which kinds of users focus on which parts of the source text. They train and test their model on the Twitter15 and Twitter16 datasets \citep{ma-etal-2017-detect} and compare the results to multiple models such as (e.g.) dEFEND \citep{10.1145/3292500.3330935} and CSI \citep{10.1145/3132847.3132877}. In their work, \citet{lu-li-2020-gcan} are able to outperform the previously best models on average by 0.16 in accuracy. Additionally, the co-attention weights can be used to explain which words and users mainly indicate fake news.
% Conclusion of that fake-news paragraph: (fokus on propagation and how that could be used in media bias detection)
%Smi
Both work show that the way news spread contains information about the content of the source. If biased and non-biased news disseminate differently, propagation-based approaches could be used to advance or complement methods used to detect media bias. Furthermore, the dual co-attention mechanism \cite{lu-li-2020-gcan} could be adapted to facilitate research in the domain of HME, e.g. which group of users focus on what part of the content.

% TODO: add transition to rumor detection: 
% - how is rumor detection similar? how is it different?
% RUMOR DETECTION
% 01_orc https://www.aclweb.org/anthology/2020.coling-main.473.pdf  
\citet{li-etal-2020-exploiting} detect rumors in social media (Twitter) based on the tree-like conversation structure, i.e. who replies whom. 
They argue that the conversation itself provides clues as to the truthfulness of the source, and that exploring these answers can help identify rumors early on. 
Using the Pheme 2017 \citep{DBLP:journals/corr/ZubiagaLP16} and Pheme 2018 \citep{10.1371/journal.pone.0150989} datasets, the authors first use a BiLSTM to generate a tweet representation and then capture the relationship between the tweets in a graph where replies are represented by edges. 
\citet{li-etal-2020-exploiting} then create a GNN and report that their model outperforms competitors in all four metrics accuracy, precision, recall and F1, including a fine-tuned BERT and the state-of-the-art model RDM \citep{zhou-etal-2019-early}. 
%Finally, the authors conclude that information propagation using textual features and the conversation structure yield better results. 
% RUMOR DETECTION is risky
% 04_orc https://www.ijcai.org/Proceedings/2020/0197.pdf  
Even though GNN-based approaches are successfully used for classification tasks in social networks \citep{li-etal-2020-exploiting, DBLP:journals/corr/abs-2007-03316}, \citet{ijcai2020-197} argue that using these such strategies in rumor detection is risky. 
Rumors could use camouflage strategies such as connecting the posting user to high-credit users, changing comments to simulate more support and other similar disguising mechanisms. 
Therefore, the authors explore several camouflage methods and develop a graph adversarial learning framework to increase the models robustness against perturbation issues. 
They evaluate their model on a chinese \citep{DBLP:journals/corr/abs-1811-04175} and an english \citep{DBLP:journals/corr/ZubiagaLP16} dataset. 
Furthermore, \citeauthor{ijcai2020-197} compare their results to several baseline models, such as GLAN \citep{DBLP:conf/icdm/YuanMZHH19} and GAN-GRU \citep{DBLP:conf/www/Ma0W19} and are able to significantly outperform these models. 
According to the authors, this indicates that taking into account camouflage mechanisms indeed increases the chance of detecting rumors. 
% TODO: add conclusion of that paragraph: How is that beneficial for media bias detection? is it beneficial at all? Or is it just an interesing aspect that is nice to know?

% Intro: explain, why this tasks (multi target dependent sentiment classification) benefits media bias detection: 
% - target dependent sentiment classification can be a first step in identifying bias
Bias can be induced in many different ways inter alia through word choice, e.g. using inflammatory or neutral wording to describe an event or a specific target (see section \ref{media bias}). 
Being able to identify target-dependent sentiment in sentences can hence be a valuable first step in identifying media bias.
% MULTI TARGET DEPENDENT SENTIMENT CLASSIFICATION
% 05_orc https://www.aclweb.org/anthology/2021.eacl-main.142.pdf -- wip (jerome)
NewsMTSC \citep{hamborg-donnay-2021-newsmtsc} is a dataset for (multi-)target-dependent sentiment classification that contains 11,3k labeled sentences. 
authors randomly select articles from two datasets, POLUSA \citep{10.1145/3383583.3398567} and Bias Flipper 2018 \citep{chen-etal-2018-learning} and keep only sentences that contain meaningful target mentions. 
Additionally, they filter these in order to obtain a set of optimal candidates and address class imbalance. Each sentence is labeled by five crowdworkers. 
Their answers are then consolidated restrictively to ensure the quality of the resulting dataset. 
Furthermore, \citet{hamborg-donnay-2021-newsmtsc} propose a classifier, GRU-TSC,  that incorporates contextual embeddings of the sentences and representations of external knowledge sources. In their work, \citet{hamborg-donnay-2021-newsmtsc} compare GRU-TSC to several models like SPC-Bert \citep{devlin-etal-2019-bert}, TD-Bert \citep{8864964} and LCF-Bert \citep{app9163389}, test it on three commonly used datasets and report an improved F1-score of 1.3pp over the state-of-the-art.
% TODO: Conclusion: 

% MEDIA BIAS DETECTION
% 06_orc https://arxiv.org/pdf/2005.04518 
% \citet{baly-etal-2020-written} try to improve media bias detection by combining the following features which we describe below: (i) the content of articles, (ii) information about the respective audience and (iii) information about the medium itself. They extract various linguistic features from articles as well as embedding features to represent (i) the content of articles. Additionally, the authors process speech segments from videos posted on the outlets YouTube channel and extract features from the mediums Twitter account such as geographical location, verification status and the profiles description. To model (ii) information about the mediums audience, they analyze the self-description of those Twitter users that follow the medium, use the Facebook Marketing API to retrieve an estimate of the outlets audience and obtain metadata from YouTube, such as views and likes, to model audience interaction. In their prior work, \citet{baly-etal-2018-predicting} showed that using an outlets Wikipedia page can help predicting its credibility and potential political bias. The authors therefore encode the outlets Wikipedia page to obtain (iii) information about the outlet itself. 
% \citet{baly-etal-2020-written} evaluate the influence of the individual features 
%as well as the possible combinations
% and conclude that, while the articles contents matter most, adding information from additional sources like Wikipedia, the outlets Twitter account or their audience leads to substantially better results. The authors report an F1-score of 84.77, an improvement of approximately 12 percentage points compared to their previous work. 

% MEDIA BIAS DETECTION
% 07_orc https://arxiv.org/pdf/2010.10652
% \citet{chen-etal-2020-analyzing} study unfairness, political bias and non-objectivity in news articles at different aggregation levels, from single words to the entire article discourse. The authors scrape labeled articles provided by Allsides\footnote{As described in XXX} and Ad Fontes media\footnote{As described in XXX} and combine them into a final corpus consisting of 6964 articles from 41 media outlets. They create three identical recurrent neural networks (RNNs) with gated recurrent units (GRUs) and a binary classification layer for each classification task. Furthermore, they perform a feature analysis to determine those words, sentences and paragraphs that mainly introduce bias by iteratively removing text segments from the articles. \citet{chen-etal-2020-analyzing} find that articles usually start neutrally but introduce bias in the latter sentences and paragraphs. At the word level, negative emotions, anger and affect correlate with political bias.

% TODO: Intro to that paper
% - focus on the value of unsupervised learning
% - maybe refer to distant supervised papers
% - explici labeling is both expensive and prone to errors as crowdworkers will introduce additional bias
% 08_orc https://arxiv.org/pdf/2104.08829.pdf
% - Also, graph modeling and learning is very new in the area. We could add one or two sentence about why the auto-encoders, who usually suck (Actually thats published nowhere but we tried it last year and it sucked bit time :-D) at bias detection, work well here.
% - Also, now that I read it again, I would probably add a short definition of what they identify as polarization/framing.
SLAP4SLIP (Sparse language properties for social link prediction) is a general framework developed by \citet{hofmann2021modeling} that detects polarized concepts in social networks without explicitly labeled data. 
Using predefined linguistic features \textit{l}, SLAP4SLIP detects how concepts are depicted and discussed in different parts of a social network. The choice of these linguistic features \textit{l} is crucial and heavily depends on the application. 
Hence, with proper adjustments, their framework can be used in many applications. 
The authors also introduce a new Reddit Politosphere Dataset, consisting of comments from 606 political subreddits posted between 2008 and 2019. 
Each year is represented as a social network, where nodes are subreddits and the edges are weighted according to the number of users that posted frequently in both subreddits. 
The authors deploy their minimally supervised method to extract features representing both, ideologically driven agenda setting and framing in subreddits. 
They train various graph auto-encoders (GAEs) and find that modeling agenda setting and framing together is best suited to identify ideological polarization. Finally, by examining the weight distribution, they analyze how concepts are polarized, e.g. if agenda setting or framing prevail, or along which moral foundations framing occurs. 
% TODO: conclusion of that paper
% - stress once again, why unsupervised learning could help here

%  Intro to neutralization
% - simply expose to opposing news may have a negative effect
% -> Hence use other methods like neutralization
Even though media bias detection can be seen as a discipline of its own, a more holistic perspective reveals that merely detecting bias and exposing users to opposing angles does not necessarily mitigate its negative psychological and ultimately societal consequences. 
As discussed in section \ref{psych}, disrupting selective exposure does not necessarily lead to a less biased perspective; it may even have the opposing effect. Some researchers therefore go a step further and explicitly change the content of an article to a more neutral wording.
% NEUTRALIZATION
% 09_orc https://arxiv.org/pdf/2104.00336  
\citet{DBLP:journals/corr/abs-2104-00336} propose neutralized article generation as a new task in the domain of media bias mitigation. They combine left-winged and right-winged articles into a single, newly generated neutral article. The authors define neutralization as a two part optimization issue, where the following two aspects are equally important. The newly generated article has to retain as much information as possible while simultaneously eliminate as much bias as possible. Therefore, \citet{DBLP:journals/corr/abs-2104-00336} introduce a new metric that tries to maximize information recall and minimize bias. Additionally, they introduce a new dataset, NEUtralize NeWS (NEUWS), consisting of 580 article triplets (left-winged, right-winged, neutral) with 1740 full articles. They perform experiments on various transformer-based architectures and conduct A/B testing to verify that their proposed metric matches human judgment. Their results show significant improvements in terms of both, information recall and bias reduction that also align with human judgement. 
% NEUTRALIZATION
% 10_orc https://dl.acm.org/doi/10.1145/3449139
Similarly, \citet{10.1145/3449139} introduce a transformer-based encoder-decoder framework, that first identifies polar sentences and then regenerates them neutrally or with the opposite polarity. The first component of their model, the Polarity Detector, builds upon the powerful language understanding capabilities of XLNet \citep{NEURIPS2019_dc6a7e65}, by adding an additional classification layer to detect liberal, neutral and conservative sentences. The encoder then receives not only the original sentence, but also the polarity label. By adding a binary classification layer on top of the encoder, the latter becomes a discriminator, effectively altering the models structure to a GAN network, where the decoder acts as a conditional generator. In addition to their model, \citet{10.1145/3449139} create a new annotated dataset that contains over 360k articles from 13/ 22 outlets. The benchmark dataset that until then represented the state-of-the-art only contains 6447 news articles \citep{chen-etal-2018-learning}. The authors are able to outperform prior work \citep{chen-etal-2018-learning, DBLP:journals/corr/abs-1911-09709} by 10\%. However, these studies only applied flipping of political polarity to headlines. To further test their results, the authors conduct an online experiment and find that their model indeed is able to reverse and neutralize effectively, while still preserving content and maintaining readability fluid.

% TODO: outcome of that subsection: story should be that 
% - by looking at related disciplines we can learn
% - by looking at methods used in similar tasks we can benefit from insights 
% - media bias detection itself is helpful but media bias mitigation is the ultimate goal/ outlook -> automatic neutralization of articles
Scientists usually conduct their research within a narrow framework. 
This makes the research process easier as it facilitates problem definition and helps keeping the overview. 
However, by looking at related disciplines we can gain valuable insights that can stimulate research into detecting media bias. 
The collection of relevant graph data from social media in combination with propagation-based methods could 

%Maybe: https://dparra.sitios.ing.uc.cl/pdfs/PRE_PRINT_GENE_Graph_generation.pdf
%Maybe: https://dl.acm.org/doi/pdf/10.1145/3340531.3412046?casa_token=AqQoLilE3SoAAAAA:_ljsesU4Iv75sinrOKg7zX-zhSXAjNxLcmIQzUx55WZ0knbzyjB4kKj62ydppQJv3qEh_Rzl8Mdy

==> Chapters/archive/CS_methods_before_restructure.tex <==
%Link to ToDo / Question Board: https://docs.google.com/spreadsheets/d/1GsgFbqRvgUeomS4-MlaWHPORbJ-Op3QVr0En9oLmVck/edit#gid=0
%left fixed width:
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
 
% center fixed width:
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
 
% flush right fixed width:
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

%What is the structure of the different categories? 
%Explain what it is, mention workflow?
%
% datasets
    % granularity of datasets
    % what datasets are they /classification of datasets
    % dataset generation
    % semi-supervised learning, distant supervision, pseudo labelling
%
% Conclusion of the CS methods part?
%_______________________________________________________________________________________
%Feedback Terry
%check out this survey for structure, they define "persepctives" they explore: https://aclanthology.org/2021.emnlp-main.414.pdf
%then explain Figure - the hierarchy/taxonomy we are proposing

\section{Computer Science Research on Media Bias} \label{csmethods}
Computer science methods fulfill two major purposes in media bias research: firstly, to analyze media bias, and secondly, to mitigate and debias texts.
Detecting bias is a prerequisite for either of the two application tasks \cite{raza_dbias_2022}.
Further, bias detection systems could be used to check computer-generated texts for bias.
In addition to the media bias framework, we contribute a structured comprehensive overview of the use of computer science methods in media bias research in recent year, based on a systematic literature review. 
To the best of our knowledge, this is the most comprehensive effort on surveying media bias so far \cref{sec:rel_lit}. 
However, for capturing the state of media bias research and the identification of research trends and gaps it is critical.

\subsection{Classification of Computer Science Methods for Media Bias Detection}\label{sec:classification_csMethods}
Our analysis shows that media bias detection methods use approaches ranging from traditional, count-based NLP methods and simple machine learning techniques, often used by social sciences (e.g., \citet{kroon_guilty_2021}), to complex computer science frameworks that combine different advanced classification approaches (e.g., \citet{Hamborg_2021}), to innovative graph-learning-based approaches (e.g., \citet{hofmann_modeling_2021}).

Since the approaches of computer science to media bias detection presented in this section are diverse, we structured them according to the type of methodology used. 
Therefore, we introduce a classification system, depicted in figure~\ref{fig:cs_classification}. 
The main separation is made between traditional natural language processing (\gls{tNLP}) approaches, machine learning approaches, and  graph-based approaches. 
Traditional natural language processing approaches are commonly used in social sciences and due to their effectiveness for similar tasks, we report on them in \cref{sec:tNLP}. 
They include primarily count-based techniques supported by lexical resources. 
We divide the diverse category of machine learning based approaches further into techniques leveraging artificial neural networks or deep learning, and other machine learning techniques. 
Since transformer-based techniques are not only a recent trend in machine learning, but also one of the more frequently used approaches (compare section \ref{sec:}), we further subdivide the deep learning category into transformer-based and non-transformer-based approaches.
%-   explain figure \ref{fig:cs_classification}
% To Do: Better Figure, then describe

\begin{figure}[h]
    \caption{Classification of computer science methods for media bias detection we use in our analysis. Publications can employ multiple approaches and thus appear in multiple categories. }
    \label{fig:cs_classification}
    \includegraphics[width=\linewidth]{figures/cs_methods_classification.png}
\footnotesize
\end{figure}

\subsection{Results of Literature Review}

Table \ref{table:csmethods1} structures the findings of our literature review described in \ref{sec:methodology} by year and category of employed computer science method. 
Overall, transformer based approaches show up most frequently, being incorporated in almost half of the approaches.

\begin{table}[H]
\begin{tabular}{L{2cm}|L{2cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|l}

 & 2019 & 2020 & 2021 & 2022 & total \\\hline
other ML techniques & \cite{ anthonio_team_2019, dinkov_predicting_2019, baly_multi-task_2019, sapiro-gheiler_examining_2019} & \cite{ leavy_uncovering_2020, bourgeois_selection_2018, stefanov_predicting_2020, mokhberian_moral_2020, alzhrani_ideology_2020, kameswari_enhancing_2020, ganguly_empirical_2020, chen_detecting_2020, shahid_detecting_2020, van_den_berg_context_2020} & \cite{ orbach_out_2020, Spinde_2021f, cuellar-hidalgo_luc_2021, zhou_hidden_2021, rao2021gender, Spinde_2021a, bauer_analyzing_2021, krommyda_experimental_2021} &  & 23 \\\hline
non-transformer-based & \cite{ han_fallacy_2019, hube_neural_2019, bordia_identifying_2019, ananya_genderquant_2019, gangula_detecting_2019} & \cite{ baly_we_2020, field_unsupervised_2020, xiao_timme_2020, cruz_document_2020, hube_methods_2020, mathew_hatexplain_2020, lazaridou_discovering_2020, jiang_comparing_2020, webson_undocumented_2020, chen_analyzing_2020} & \cite{ ruan_pseudo-labelling_2021, sinno_political_2022, cuellar-hidalgo_luc_2021, gerald_ki_wei_huang_hyperpartisan_2021, ruan_bias_2021, Spinde_2021a, krommyda_experimental_2021} & \cite{ liu_political_2021, fagni_fine-grained_2022} & 25 \\\hline
traditional NLP techniques & \cite{ wevers_using_2019, badjatiya_stereotypical_2019, taylor_illegal_2019, sapiro-gheiler_examining_2019, cornelissen_computational_2019} & \cite{ leavy_uncovering_2020, zahid_modeling_2020, niven_measuring_2020, ferrer_discovering_2020, papakyriakopoulos_bias_2020, de_arruda_analysing_2020, aires_information_2020, mendelsohn_framework_2020} & \cite{ koprinska_media_2020, dalonzo_machine-learning_2021, Spinde2021, kroon_guilty_2021, Kwak_2021, dacon_does_2021, sales_assessing_2021} &  & 20 \\\hline
transformer-based & \cite{ han_fallacy_2019, gao_target-dependent_2019, dinkov_predicting_2019, fan_plain_2019, pryzant_automatically_2019} & \cite{ baly_what_2020, baly_we_2020, li_using_2021, pant_towards_2020, stefanov_predicting_2020, PoliBert20, mokhberian_moral_2020, bhardwaj_investigating_2021, tran_how_2020, mathew_hatexplain_2020, mozafari_hate_2020, chen_detecting_2020, van_den_berg_context_2020, jiang_comparing_2020, kwak_systematic_2020} & \cite{ huguet_cabot_us_2021, blackledge_transforming_2021, kameswari_towards_2021, madanagopal_towards_2021, ruan_pseudo-labelling_2021, sinno_political_2022, orbach_out_2020, hamborg_newsalyze_2021, Spinde2021f, hofmann_modeling_2021, zhou_hidden_2021, sinha_determining_2021, he_detect_2021, ruan_bias_2021, bauer_analyzing_2021, spinde_interdisciplinary_2021, liu_transformer-based_2021} & \cite{liu_politics_2022, lee_neus_2022, spinde_exploiting_2022, raza_dbias_2022, krieger_2022} & 46 \\\hline
graph-based &  & \cite{ stefanov_predicting_2020, chen_neutral_2021, chitra_analyzing_2020} & \cite{ zhou_uncovering_2021, hofmann_modeling_2021, villa_echo_2021, guimaraes_characterizing_2021} & \cite{ guo_modeling_2022} & 8  \\\hline
total & 17 & 41 & 34 & 8 & 
\end{tabular}
\caption{Results of literature study on computer science methods used for media bias detection.} 
\label{table:csmethods1}
\end{table}

\begin{figure}[h]
    \caption{Overview of relevant publications per category and year. Publications can appear in multiple categories.}
    \label{fig:cs_classification}
    \includegraphics[width=\linewidth]{figures/publications_per_year.png}
\footnotesize
\end{figure}

%_______________________________________________________________________________________

\subsection{Analysis of Categories for Media Bias Detection}\label{sec:lit_rev}
In the following section we present an analysis of the introduced categories and important publications, starting with traditional natural language processing techniques, followed by transformer-based models, non-transformer-based models, other machine learning techniques and lastly, graph-based approaches.

%_______________________________________________________________________________________

\subsubsection{Traditional Natural Language Processing Techniques}\label{sec:tNLP}cs_methods_classification
The traditional natural language processing category includes all publications that identify media bias using techniques not based on machine learning or graph-based-approaches. 
Most \gls{tNLP} techniques employed for media bias detection are count-based. 
Recently however, word embeddings have been used as a means of representing texts and analyzing the associations and inherent biases \citet{caliskan_semantics_2017}.
We include the 'traditional' in the name of the category to differentiate it from machine-learning techniques and similar techniques.
Furthermore, techniques similar to what we label \gls{tNLP} have already been used in the field of computational linguistics in the sixties and seventies \cite{coling-1965-coling}.
Due to their explainability and proven effectiveness, \gls{tNLP} techniques are often used as a baseline to evaluate the effectiveness of new techniques (\cite{example1, example2, example3}) or the suitability of new datasets for different tasks (\cite{example1, example2, example3}). 
Further, social sciences use them increasingly due to the accessibility and ease-of use \cite{kroon_guilty_2021}.

%_______________________________________________________________________________________

\textbf{Count-based Approaches.}
The majority of recent applications of \gls{tNLP} techniques are primarily count-based. 
\cite{leavy_uncovering_2020} investigate gender bias in Irish newspapers in terms of various discriminative factors. 
In addition to investigations that employ machine learning techniques, they detect coverage bias towards female politicians using count-based \gls{tNLP} approaches. 
\citet{niven_measuring_2020} measure texts' alignment to authoritarian state media. 
They use a count-based methodology leveraging LIWC \cite{pennebaker01} categories for topical categorization. 
In \citet{dacon_does_2021}, the authors present a study on gender bias in news abstracts using various \gls{tNLP} techniques in conjunction with related concepts such as sentiment analysis.
\citet{de_arruda_analysing_2020} use a count-based approach in an outlier detection framework for the detection of selection-, statement- and coverage bias.
\citet{koprinska_media_2020} use different count-based \gls{tNLP} techniques and them to find the most effective set of techniques for media bias detection. 
They evaluate count-based metrics for bias- and sentiment lexicons, word embeddings, and general TF-IDF measures.
Using a mix of different \gls{tNLP} techniques, \citet{zahid_modeling_2020} investigate coverage bias and statement bias towards certain topics and entities introducing the concept of absolute and relative media bias. 
\citet{dalonzo_machine-learning_2021} present a singular value decomposition approach that predicts which newspaper published a given article, based on word frequencies. 
The system produces a conditional probability distribution that allows for automatically projecting newspapers and phrases into a bias space. 
\citet{taylor_illegal_2019} present the Newsalyze pipeline of mostly count-based NLP techniques that aims to mimic human annotation to investigate framing bias \footnote{The authors use the term "bias by word choice".}. 

%_______________________________________________________________________________________

\textbf{Word Embedding Based Techniques.}
The other category of frequently used \gls{tNLP} techniques detects media bias by deriving word associations via word embeddings. 
Although we exclude publications that focus on investigating bias in word embeddings, we include work that identifies bias in word embeddings in order to investigate biases in the texts used to create the embeddings.
The majority of word embedding based techniques can directly or indirectly be traced back to \cite{caliskan_semantics_2017} and their word embedding association test (WEAT).
\citet{ferrer_discovering_2020} investigate various aspects of linguistic and gender bias on Reddit using a technique similar to WEAT. 
They further investigate biases using count-based approaches and sentiment analysis. 
%todoSmi see comment, the cite is correct
In \citet{spinde2021}, the authors train two word embedding models on slanted news corpora to identify strongly biased words. 
\citet{wevers_using_2019} published an investigation of gender bias in dutch newspapers from 1950-1990. 
They measure the distance of ``three sets of targets words"\cite{wevers_using_2019} to two gender-representative vectors. 
The vectors are built on the average of lists of ``gender words"\cite{wevers_using_2019}, for example ‘man’, ‘his’, ‘father’ and other similar words for the male vector. 
Similarly, \citet{papakyriakopoulos_bias_2020} used word embedding associations to compare gender bias in Wikipedia and social media texts. 
\citet{kroon_guilty_2021} likewise analysed implicit associations using word embeddings to detect racial bias\footnote{The authors use the term ``ethnically stereotyped bias"}.
\citet{badjatiya_stereotypical_2019} base their method on the idea of bias sensitive words and their identification and proposing debiasing strategies. 
They employ multiple methods: aside from machine learning techniques, they employ \gls{tNLP} techniques, such as count-based-probabilistic metrics (f.e. Skewed Predicted Class Probability Distribution), and embedding-based approaches.
\cite{mendelsohn_framework_2020} investigate the development of dehumanization towards the LGBTQ community in New York Times news articles from 1986 to 2015 by means of primarily embedding-based \gls{tNLP} techniques. 
%_______________________________________________________________________________________
\citet{Kwak_2021} present an approach to bias detection based on word embeddings, that differs from the other publications in this section. 
First, they define a range of microframes that span an axis in the vector space of embeddings, for example along the axis of 'depressing' and 'cheerful'. 
Then, their system classifies texts along these microframes.
\citet{sales_assessing_2021} use a mixed methodology based on word embeddings that includes lexicon translation, and document similarity measures to detect subjectivity bias.

%_______________________________________________________________________________________
%_______________________________________________________________________________________
%_______________________________________________________________________________________

\subsubsection{Machine Learning - Transformer-Based Models}\label{sec:tbML}
Next, we summarize the research that uses transformer-based models to detect media bias.
Transformer-based models saw an ongoing rise in popularity after their introduction in 2017 \cite{Transformer2017} which reflects in the final table \ref{table:csmethods1}.
Most publications implement and evaluate multiple transformer models. 
Especially due to the novelty of transformers, best practices in terms of what transformer works best for which task are mostly still to be determined. 
Therefore, we structure this overview by type of bias, to facilitate evaluating the use of different transformers for the identification of different types of media bias.
In table \ref{table:transformers} we provide an overview on the types of media bias transformer-based research focuses on.

Transformers are sequence transduction models that replace recurrent layers in encoder-decoder architectures with multi-headed self-attention \cite{Transformer2017}.
Pre-trained language models like BERT are popular because of their accessibility, i.e. on Huggingface\footnote{https://huggingface.co/bert-base-uncased}, and the possibility to train online.
Further, they can be fine-tuned with specific domain-specific datasets without training from scratch, saving time and computational resources.
What makes them powerful is their universal architecture that is able to capture dependencies of different ranges, with the slight downside of over-fitting when data is limited \cite{linSurveyTransformers2021}.

Researchers frequently use transformer-based methods to detect linguistic bias, or political ideology (compare table \ref{table:transformers}).
Most commonly, researchers use BERT or BERT-based models, eg. RoBERTa \cite{Spinde_2021f, madanagopal_towards_2021, huguet_cabot_us_2021, hamborg_newsalyze_2021, zhou_hidden_2021, raza_dbias_2022, van_den_berg_context_2020, krieger_2022}, DistilBERT \cite{blackledge_transforming_2021, spinde_exploiting_2022, raza_dbias_2022}, or ALBERT \cite{kameswari_towards_2021}, mostly with an encoder only architecture and bias-specific pre-training.
BERT-based models are applied to detect media bias in languages beside English, like Korean ((Kor)BERT) \cite{han_fallacy_2019}, Indian (IndicBERT) \cite{kameswari_towards_2021} or finetuning BERT on African American \citet{Mozafari_2020}.
Additionally, some works compare the performance of other transformer models, e.g. T5 \cite{krieger_2022}, BART \cite{lee_neus_2022, he_detect_2021}, ELECTRA \cite{Spinde_2021e} or XLNet \cite{liu_transformer-based_2021}.
An established approach is creating bias-specific datasets, testing the performance of the most popular, fine-tuned out-of-the-box models, and comparing F1-scores to baselines of traditional NLP methods (e.g. \cite{Spinde_2021e, Hamborg_2021, pant_towards_2020, Gao_2019, krieger_2022}).
%
%Conclusion from transformers here?
After examining the corpus of papers we conclude that BERT and RoBERTa outperform traditional NLP methods and other transformers, e.g. \cite{Spinde_2021e}.
Further, including metadata or contextual information improves accuracy and might lead to increased classification performance, e.g. \cite{dinkov_predicting_2019}.
%
\begin{table}[H]
\begin{tabular}{L{4cm}|L{10cm}}
Type of Bias
& Paper 
\\\hline
Linguistic Bias
&   \cite{Spinde_2021e, raza_dbias_2022, baly_what_2020, huguet_cabot_us_2021, kameswari_towards_2021, orbach_out_2020, hamborg_newsalyze_2021, mathew_hatexplain_2020, sinha_determining_2021, ruan_bias_2021, pryzant_automatically_2019, bauer_analyzing_2021, liu_transformer-based_2021, krieger_2022, blackledge_transforming_2021, madanagopal_towards_2021, pant_towards_2020, spinde_exploiting_2022, fan2019a, jiang_comparing_2020}    
\\\hline
Framing Bias               
&      \cite{kwak_systematic_2020, hofmann_modeling_2021, mokhberian_moral_2020, Spinde_2021e, spinde_exploiting_2022, hamborg_newsalyze_2021} 
\\\hline
Stance Detection of Political Ideology         
&      \cite{liu_transformer-based_2021, mokhberian_moral_2020, PoliBert20, sinno_political_2022, liu_politics_2022, dinkov_predicting_2019, han_fallacy_2019, baly_we_2020, ruan_pseudo-labelling_2021, lee_neus_2022, chen2020detecting, fan2019a, stefanov_predicting_2020} 
\\\hline
Reporting Level Bias       
&       \cite{tran_how_2020}
\\\hline
Spin/Informational Bias    
&       \cite{van_den_berg_context_2020, fan2019a, chen2020detecting}
\\\hline
Gender Bias                
&       \cite{Mozafari_2020, he_detect_2021}
\\\hline
Racial Bias                
&       \cite{Mozafari_2020, he_detect_2021}
\\\hline
Sentiment Analysis         
&      \cite{Gao_2019, Hamborg_2021}
\\\hline
Unreliable / Fake News
&       \cite{zhou_hidden_2021}
\end{tabular}
\caption{Classification into categories of media bias in transformer-based research} 
\label{table:transformers}
\end{table}

\textbf{Linguistic Bias.} 
Most research focuses on detecting linguistic bias.
Worth mentioning is the work of \citet{Spinde_2021e} as their classifier detects bias by word choice following a distant supervision approach with BERT, outperforming RoBERTa.
With their dataset BABE \cite{Spinde_2021e}, which was annotated by trained experts and is the largest regarding bias by word choice, they achieve state-of-the-art performance, concluding that transformers outperform comparable algorithms.
%\citet{krieger_2022} ????
Contrasting, \citet{huguet_cabot_us_2021} achieve the best performance on their Us vs. Them dataset with RoBERTa.
\citet{sinha_determining_2021} also fine-tune BERT with a collected corpus and contextual embeddings.
Additionally, they parse sentences through a GCN model with an additional layer of BiLSTM to make use of structural information.
\citet{raza_dbias_2022} propose a four phase pipeline with a detection phase (DestillBERT), recognition phase (RoBERTa), bias masking phase, and a debiasing phase.
The system detects biased words, masks them, and suggests a set of sentences with new words that are bias-free or less biased.
\citet{pryzant_automatically_2019} detect and automatically transform inappropriately subjective texts into a neutral point of view.
Their concurrent system uses a BERT encoder to identify subjective words as part of the generation process, and a join embedding through which the LSTM-based classifier can edit the hidden states of the encoder.
%---------------------------------------

\textbf{Political Stance Detection.} 
The second most researched classification problem is political stance detection, an umbrella term that describes means of identifying linguistic biases in order to identify authors' political biases.
\citet{sinno_political_2022} study the ideology of specific policies under discussion, and introduce the first diachronic dataset of news articles annotated by trained political scientists and linguists at the paragraph-level.
Their fine-tuned BERT model performs best.
\citet{dinkov_predicting_2019} integrate audio data, videos, metadata, and subtitles in their multimodal dataset.
In their application, combining text analysis with BERT, including metadata, and integrating the audio data with open SMILE, resulted in the highest accuracy.
%---------------------------------------

\textbf{Framing Bias.} 
Regarding the investigation of framing bias, \citet{mokhberian_moral_2020} use BERT with tweet embeddings and an intensity score for moral frames classification, based on the moral foundation theory.
\citet{kwak_systematic_2020} propose a similar, BERT-based method for performing sociological frame analysis.
\citet{hamborg_newsalyze_2021} propose a system for bias identification which proceeds to create bias-sensitive visualizations to communicate bias.
For preprocessing, they use CoreNLP, and then perform a target concept analysis with context-driven cross-document coreference.
A RoBERTa-based neural model performs the frame identification and afterwards groups similarly slanted articles with Grouping-MFA and Grouping-ALL.
\citet{lee_neus_2022} propose a system for framing bias detection and neutral summary generation from multiple news headlines of varying political leanings to facilitate balanced and unbiased news reading.
They perform multi-document summarization (MDS), multi-task learning with two tasks and use BART for the text generation
%---------------------------------------

\textbf{Spin/Informational Bias.}
\citet{fan2019a} investigate lexical and informational bias with BERT on their BASIL dataset, which \citet{van_den_berg_context_2020, liu_politics_2022, sinha_determining_2021} also use in their research.
\citet{van_den_berg_context_2020} fine-tune RoBERTa to a context-inclusive model, exploring neighboring sentences, the full article, articles on the same event from other news publishers, and articles from the same domain.
Their model is domain-and-task-adapted for informational bias detection on the BASIL corpus.
Interestingly, integrating event context improves classification performance.
%---------------------------------------

\textbf{Racial/Group Bias.}
For group bias detection, \citet{he_detect_2021} present their DEPEN approach that detects biased writing styles with a fine-tuned BERT model.
Afterwards, they use BART to debias and rewrite the sentences.
%---------------------------------------

\textbf{Sentiment Analysis.}
We exclude general sentiment analysis but include papers that use sentiment analysis to detect media bias.
\citet{huguet_cabot_us_2021} investigate populist mindsets, social groups, and related typical emotions using RoBERTa fine-tuned on their populist attitude dataset.
Similarly, \citet{Gao_2019} implement three target-dependent variations of the BERT-based model.
\citet{Hamborg_2021} apply target-dependent sentiment classification (TSC) with BERT and a BiGRU. They propose a classifier, GRU-TSC, that incorporates contextual embeddings of the sentences and representations of external knowledge sources. 
%Their NewsMTSC dataset consist of 11,3k labeled sentences.
%---------------------------------------

\textbf{Other}
A special case intersecting with media bias detection is the detection of unreliable news that \citet{zhou_hidden_2021} detect with RoBERTa.
Further, they propose ways to minimize selection bias in the creation of datasets.
%_______________________________________________________________________________________
%_______________________________________________________________________________________
%_______________________________________________________________________________________
\subsubsection{Machine Learning - Non-Transformer-Based Models}\label{sec:ntbML}
%\paragraph{Summary: what does this category contain?}
Although transformer-based approaches are popular, other deep learning approaches to bias identification are still used frequently. 
One supposed reason for that is that before transformers, the top-performing models were deep neural networks.
Therefore, non-transformer-based models serve as the ideal baseline.
If a publication's main contribution is not the model itself, but instead the dataset (as in \cite{baly_we_2020, sinno_political_2022, ruan_bias_2021, lazaridou_discovering_2020}), or the evaluation of disruptively new \cite{chen-etal-2020-analyzing, gangula_detecting_2019} or combined approaches \cite{Hamborg_2021}, comparability is more important than effectiveness. 
In this section, we structure the various publications in which non-transformer-based deep learning are used for bias identification by their type of application. 

\textbf{Non-Transformer-Based Models as a Baseline.}
\citet{baly_we_2020} is one of the publications, in which non-transformer-based models serve as a baseline.
The main contribution of \citet{baly_we_2020} is the construction of a dataset and testing an evaluation split, where media sources appear in either training, validation, or the testing dataset.
They also evaluate the performance of an LSTM network model and a transformer-based BERT approach.
\citet{han_fallacy_2019} use BERT-based classifiers to detect political leaning of short comments. 
They use TextCNN as a non-transformer-based baseline model to compare the results of their BERT-based models to.
\citet{sinno_political_2022} present a manually annotated dataset and their studies on ideological/stance bias in news articles. 
Aside from multiple BERT-based approaches to classification, they use a 2-layer bidirectional LSTM for ideology prediction, that was outperformed by all transformer based systems.

\textbf{Political stance detection.}
Of all types of media bias researched using deep learning, political stance, as defined in \cref{sec:tbML} as political ideology classification based on linguistic bias detection, especially in the form of hyperpartisan news detection, is the most commonly analyzed.
The latter is promoted by the SemEval2019 hyperpartisan news detection task \cite{kiesel-etal-2019-semeval}, which inspired many publications, both in participation and using the dataset.
``Hyperpartisan news is news that takes an extreme left-wing or right-wing standpoint"\cite{kiesel-etal-2019-semeval} and thus represents an as pect of the political ideology classification presented in section \ref{sec:framework}.
The approach of \citet{jiang-etal-2019-team} performed best in the task.
It leverages CNN along with batch normalization and ELMo embeddings. 
\citet{jiang_comparing_2020}, in a follow up publication to \cite{jiang-etal-2019-team}, incorporate LDA distributions with different approaches to hyperpartisan news detection. 
They use CNN, RNN and a transformer encoder approach as well as two more elaborate hierarchical approaches, ELMo sentence representation convolutional network (ESRC) and hierarchical attention network (HAN) with and without LDA topic modeling. 
Their results suggest, that in most cases, LDA topic modeling improves the effectiveness of the methods, and hierarchical models outperform non-hierarchical models, despite the differences being minute.
\citet{webson_undocumented_2020} present another study based on the SemEval2019 hyperpartisan news detection task. 
In contrast to other works based on the dataset provided for this task, their work does not directly encompass bias detection. 
Rather, they focuses on decomposing pretrained embeddings into separate denotation and connotation spaces and thus identifying biased words in a very descriptive manner.
Although their primary goal is to make the embeddings better reflect the implied meaning of words, the discrepancy between denotation space and pretrained embeddings reflects partisanship. 
\citet{cruz_document_2020} use different machine learning approaches (RNN, CNN, BiLSTM/BiGRU, and the attention-based approaches AttnBL as well as Hierarchical Attention Network (HAN)) to detect hyperpartisanship in the SemEval 2019 dataset.
They evaluate the effects of attention mechanisms and embeddings based on different granularities, token- and sentence wise, on the effectiveness of the models. 
As one of the more recent publications that tried to improve on the classification results of the task, \citet{ruan_bias_2021} try to improve on the performance of previous classification attempts.
Their approach focuses on introducing methods for generating additional data.
First, they present two approaches for pseudo-labelling, overlap-checking
and meta-learning. 
Then, they introduce a (sentence) masking method, that helps with understanding the classification by observing the change in classification outcome. 
For bias classification, they use ELMo Sentence Representation Convolutional (ESRC) Network by \cite{jiang-etal-2019-team}.
In \cite{ruan_pseudo-labelling_2021} the same authors use a ELMO based classifier along with a proposes a data augmentation method using pseudo-labelling.

Aside from partisan bias, \citet{gangula_detecting_2019} propose a headline attention network approach to bias detection in Telugu news articles. 
It leverages a bi-LSTM attention mechanism, to identify key parts of the articles based on their headlines, which are then used to detect bias towards political ideologies.
They compare the results of their approach with Naive Bayes, SVM and CNN approaches, all outperformed by the headline attention network. 

\textbf{Word Embeddings}
Changing the word embeddings used with a proven classifier is a very effective way to improve on existing machine learning based media bias detection approaches. 
Therefore, many publications focus on introducing and evaluating new word embeddings for the use in non-transformer based approaches for bias identification.
\citet{mathew_hatexplain_2020} use a CNN model trained on ELMo word embeddings to identify framing bias. 
They evaluate the effectiveness of more traditional word embeddings in comparison to the ELMo embeddings.
Furthermore, they investigate the use of frequencies of bias word from lexicons as features for the CNN.
With the goal of depolarizing political news articles, \citet{fagni_fine-grained_2022} leverage custom embeddings constructed with deep learning (CNN), that then are passed through feature compressing layers, to map Italian social media users into a 2-dimensional space. 
Using clustering, they then predict the political ideology of users.

\textbf{Other}
The fact that non-transformer-based machine learning models are proven and comparatively understood, makes them also well suited for improving or testing other componentes of bias identification pipelines.
In addition to a FastText classifier, the approach presented by \citet{lazaridou_discovering_2020} includes manual selection of training data, that contains supposedly simple and easy to understand examples for media bias. 
Their goal is to improve and quicken the models' training process. 
Aside from contributing a new media bias dataset and evaluating the effect of expert and non-expert annotators, they present a curriculum learning approach for media bias detection. 
\citet{field_unsupervised_2020} present an unsupervised approach for identifying gender bias in Facebook comments. 
They use a bidirectional LSTM to predict the gender of the addressee of facebook comments and doing so, identifying gender biases in these comments.

\textbf{Mixed Approaches}\todo{combine this subsubsection with other ML techniques?}
\citet{Hamborg_2021} use a assembled approach based on a bidirectional GRU (BiGRU) that leverages the output of three components, a pre-trained language model (BERT, RoBERTa, and XLNET), a representation of external knowledge sources (EKS), and a target mention mask, to classify the sentiment of texts.
\citet{hidalgo_luc_2021} used two approaches, one using KNN, the other a mixed approach consisting of Naive Bayes, SVM, Random Forest, GBM, Adaboost and a multi-layer perceptron for classifying texts as aggressive, gender biased or communally charged.

%_______________________________________________________________________________________
%_______________________________________________________________________________________
%_______________________________________________________________________________________
\subsubsection{Other Machine Learning Techniques}\label{sec:oML}
%\paragraph{Summary: what does this category contain?}
Aside from state-of-the art approaches that utilize transformer-based or deep learning techniques for bias detection, there are more traditional or apparently simple applications of machine learning for bias classification. 
Many employ linear discriminant analysis (LDA), support vector machines (SVM) or regression models, however, some display unique approaches. 
The main reason why, despite more effective means of bias identification being available, these comparable simple techniques are still frequently used, is to evaluate or demonstrate the applicability of new datasets for bias identification.
For this task, the classification performance is not relevant and the ease of implementation is a clear advantage.


\textbf{Application of Bias Identification for Introducing New Datasets} 
Utilizing simpler but proven bias identification methods is a reliable way of demonstrating a new datasets' usefulness and facilitate a direct comparison. 
In addition to presenting a new, manually labeled corpus on media bias by word choice, \citet{Spinde_2021f} also evaluate a range of different bias detection approaches. 
The models they use for classification (LDA, logistic regression, QDA, NB, KNN, DT, RF, SVM, XGBoost, MLP) are provided a set of linguistic features.
These feature include  POS tags, named entities (and their types), TF-IDFs, in addition to a custom, semi-automatically created lexicon of biased words, that have all been used in previous approaches to media bias detection. 
\citet{alzhrani_ideology_2020} contribute a dataset of personalized news. 
Furthermore, they evaluate a range of classifiers (Ridge classifier, nearest centroid, SVM with SDG, Naive Bayes) for political affiliation detection.
\citet{rao2021gender} investigate gender bias in their dataset of Canadian news articles. 
They employ LDA topic modelling to detect biased topic distributions for articles that contain majority male or female sources. 
\citet{kameswari_enhancing_2020} present a dataset consisting of 200 unbiased and 850 biased articles written in Telugu. 
They use NB (Bernoulli and multinomial), logistic regression, SVM, RF and MLP classifiers to evaluate the effectiveness of the addition of presuppositions as model input. 
Aside from contributing a new media bias dataset and evaluating the effect of expert and non-expert annotators, \citet{lazaridou_discovering_2020} present a curriculum learning approach to media bias detection. 
In addition to a FastText classifier, their methodology includes a manual selection of training data, that contains supposedly easy to understand examples for media bias. 
Their goal is to improve and quicken the models' training process. 
\citet{shahid_detecting_2020} research framing effects in news. 
After constructing a labeled dataset and investigating various aspects of moral framing, they train a SVM classifier to detect moral framing and comparing it to a baseline lexicon-based NLP approach.
\citet{Spinde_2021a} evaluate a dataset, which is the main contribution of the publication, by comparing different classifier for media bias detection. The models they evaluate are LR LDA, QDA, NB, SVN, KNN, DT, RF, XGBoost, as well as the best performing MLP.
\citet{ganguly_empirical_2020} investigate various biases that can appear while building a media bias dataset. 
A part of their work consists of investigating the correlation between a news articles' political bias and its media outlets' political stance.
They do so by training MNB, SVM, LR and RF models, using ground-truth labels and, in comparison, the outlets political stance as labels for their news articles.

A range of other publications include the application of non-transformer based, non-deep-learning machine learning approaches in addition to other machine learning techniques for dataset evaluation. These have been mentioned in sections \todo{add sections} \citet{dinkov_predicting_2019, mokhberian_moral_2020, leavy_uncovering_2020, zhou_hidden_2021, orbach_out_2020} 


\textbf{Innovative Applications and Mixed Approaches}
\citet{baly_multi-task_2019} present a multi-task ordinal regression framework for classifying political ideology and trustworthiness simultaneously. 
This approach is based on the assumption, that both phenomena are intertwined. 
\citet{dacon_does_2021} employ decision tree naive Bayes, support vector machine, and lasso-penalty regression models, based on bag-of-word information to classify politicians' ideological positions and their trustworthiness.
The regression model they use, copula ordinal regression (COR), is adopted from facial action detection. 
The analogy that is leveraged here is, that, similar to certain facial features, trustworthiness and ideology co-occur.
\citet{anthonio_team_2019} similarly base their work on the connection between two phenomena. They use a linear SVM with VADER sentiment scores as a feature, relying exclusively on the intensity of negative sentiment in texts to derive political ideologies expressed in texts.
\citet{cuellar-hidalgo_luc_2021} present their contribution to the ICON2021 Shared Task on Multilingual Gender Biased and Communal Language Identification \todo{reference}, in which the goal is classifying texts as aggressive, gender biased or communally charged. 
The authors used two approaches, one using KNN, while the other is a mixed approach consisting of s Naive Bayes, SVM, Random Forest, GBM, Adaboost and a multi-layer perceptron.
\citet{sapiro-gheiler_examining_2019} employ a word-count approach (bag-of-words) as a basis for various ML techniques, to rate politicians' ideological positions and their trustworthiness.

%_______________________________________________________________________________________
%_______________________________________________________________________________________
%_______________________________________________________________________________________
\subsubsection{Graph-Based}\label{sec:Graph-based}
%\paragraph{Summary: what does this category contain?}
In the following we summarize methods for media bias detection that used graph-based methods.
Often, research on fake news spreading and rumor detection leverage graph data structures that describe online social networks and interactions \cite{fakenewsGraphBased}.
We find the application of graph-based methods for media bias research in computer science to be limited, finding 8 papers in total.

%SLAP4SLIP framework probably the most interesting contribution, but hard to grasp/summarize
%I think they all used semi/unsupervised training? worth mentioning?
%The first Slap4Slip part is long, but I think it's the most noteworthy contribution. Let me know which parts I can throw out!
\textbf{Framing Bias.}
The SLAP4SLIP framework by \citet{hofmann2021modeling} detects how concepts are discussed in different parts of a social network with predefined linguistic features, graph neural networks and structured sparsity.
The authors exploit the network structure of discussion forums on Reddit without explicitly labeled data and minimally supervised features representing ideologically driven agenda setting and framing.
Training graph auto-encoders (GAEs), \citet{hofmann2021modeling} conclude that modeling agenda setting and framing together is best suited for identifying ideological polarization by examining the weight distribution.
Further, they propose the MultiCTX (Multi-level ConTeXt) model that consists of contrastive learning and sentence graph attention networks to encode three different levels of context: neighborhood-context of adjacent sentences, article-context, and event-context.
Noteworthy, their properly adjusted framework can be used in a variety of scenarios. 
%Modeling Multi-level Context for Informational Bias Detection by Contrastive Learning and Sentential Graph Network 2022!!!
\citet{guo_modeling_2022} build on \citet{hofmann2021modeling} Slap4Slip framework to detect informational bias and ideological radicalization by combining contrastive learning and sentential graph networks.
Combining it with BERT for moral foundation detection, they predict links with a graph auto encoder.

%How biased are American media outlets? A framework for presentation bias regression
Similarly, \citet{tran_how_2020} propose a framework for identifying bias in news sources.
The authors use BERTbase for an aspect-based sentiment analysis and assigns bias scores for each source with a graph-based algorithm.

\textbf{Echo Chambers.}
\citet{villa_echo_2021} apply community detection strategies and model a COVID-19 related conversation graph to detect echo chambers.
Their method considers the relationship between individuals and semantic aspects of their shared content on Twitter.
By partitioning four different representations of a graph (topology-based, sentiment-based, topic-based, and hybrid) with the METIS algorithm, followed up by qualitative methods, they assess the levels of controversy and homogeneity.

\textbf{Political Stance Detection.}
Similar to \gls{tbML} and non-transformer-based machine learning, stance detection\footnote{We define stance as political bias detection via the identification of linguistic biases, compare \cref{sec:tbML}.} is a common application of graph-based classification techniques. Four papers use graph-based methods to detect political stance by incorporating social information \cite{stefanov_predicting_2020, guimaraes_characterizing_2021, zhou_uncovering_2021, li-goldwasser-2019-encoding}.
%Uncovering Media Bias via Social Network Learning
\citet{zhou_uncovering_2021} combine network structure learning analysis and neural networks.
With their semi-supervised network Embedding Approach, the authors build a training corpus on network information including macro- and micro-network views.
To predict the labels, they employ network embedding learning and graph-based label propagation.
%Predicting the Topical Stance and Political Leaning of Media using Tweets (as feature)
By integrating graph embeddings as a feature, \citet{stefanov_predicting_2020} detect stance and political leaning of Twitter users and online media by leveraging their retweet behavior.
They use a user-to-hashtag graph and a user-to-mention graph and run node2vec afterward.
Combining BERT with valence scores achieved the best result.
%Characterizing political bias and comments associated with news on Brazilian Facebook
\citet{guimaraes_characterizing_2021} analyze news stories and political opinions shared on Brazilian Facebook.
They base their methodology on graph-based semi-supervised learning to classify Facebook pages to the political left or political right.
Utilizing audience interaction information by inferring self-reported political leaning from Facebook pages, \citet{guimaraes_characterizing_2021} use a interest graph to determine the stance considering related pages.
The authors achieved the best results from label propagation with spectral graph transducer (SGT).
%Encoding Social Information with Graph Convolutional Networks for Political Perspective Detection in News Media
\citet{li-goldwasser-2019-encoding} capture social context with a neural architecture for representing relational information
with graph-based representations and a graph convolutional network. 
They show that using social information like Twitter users that shared the article can significantly improve performance with distant and direct supervision.

\subsubsection{Other}\label{sec:other_class_techn}
\textbf{Bias in Language Models.}
Besides using language models to detect bias, bias inherent in language models is a field of concern.
\citet{nadeem_stereoset_2021} analyse stereotypical bias with the crowdsourced dataset StereoSet in BERT, GPT2, ROBERTA, and XLNET, concluding that all models exhibit strong stereotypical bias.
\citet{vig_investigating_2020} use casual mediation analysis to analyse gender bias in language models.
Their results show that gender bias effects exists in specific components of language models.
\citet{bhardwaj_investigating_2021} also analyze gender bias within BERT-layers and conclude that the layers are generally biased.

\subsubsection{Datasets}

During our review, we do not only collect methods from select papers, but also datasets. We categorize the datasets into the same concepts as given by our media bias framework, as we do with the methodologies. Overall, our review returns 116 datasets. Their assignments to the categories are shown in \todo{cref table about -- link see comment}. However, we do not evaluate dataset quality, since all datasets have very different task and quality assessment will be a project in itself\footnote{we will refer to this again in \cref{sec:discussion}}. We notice that only two out of all datasets include annotator background, and that dataset sizes are generally small (only 21 out of 116 datasets have more than 30,000 annotations). We believe that using multiple datasets can be promising for future work, and will also refer to that again in \cref{sec:discussion}. For our literature review, we mainly want to add the datasets and their statistics and tasks as a starting point for future work, without further assessment. We give a detailed overview about publications, sizes, availability, tasks, type of label, link and paper summary in the appendix uploaded to Zenodo \todo{add link and table}.

==> Chapters/archive/Labels.tex <==
%Section Labels
sec:introduction
sec:related
sec:methodology
sec:rel_lit
csmethods
sec:psychology
sec:conq
sec:discussion
sec:appendix

%Related work Labels
sec:bias
sec:framework
fig:framework
sec:linguistic_bias
sec:text_level_bias
sec:reporting_level_bias
sec:cognitive_bias
sec:related_concepts

%Methodology Labels
sec:crawl
table:searchResults (commented out)
sec:review
fig:cs_crawl
sec:review_concepts

%CS methods labels
sec:tNLP
sec:ArtifNeuNet
sec:TransformerBasedModels
tbML_pol_stance_det
sec:ntbML
sec:oML
sec:other_class_techn
sec:Graph-based
sec:other_csmethods
sec:datasets

%CS methods figures and tables
fig:cs_overview
table:csmethods1
fig:cs_classificatio (yeah theres a typo in the label)
table:datasets


%Bias example table Labels Appendix
table:categories1
table:categories2
table:categories3
table:categories4



not sure if those work in the appendix table (only one left tho):
ConnotationBias



%
%In table \ref{table:transformers} we provide an overview of the types of media bias occurring in the datasets for fine-tuning.
%\begin{table}[H]
%\begin{tabular}{L{4cm}|L{10cm}}
%%Type of Bias
%& Paper 
%\\\hline
%Linguistic Bias
%&   \cite{Spinde2021f, raza_dbias_2022, baly_what_2020, huguet_cabot_us_2021, kameswari_towards_2021, orbach_out_2020, hamborg_newsalyze_2021, mathew_hatexplain_2020, sinha_determining_2021, ruan_bias_2021, pryzant_automatically_2019, bauer_analyzing_2021, liu_transformer-based_2021, krieger_2022, blackledge_transforming_2021, madanagopal_towards_2021, pant_towards_2020, spinde_exploiting_2022, fan2019a, jiang_comparing_2020}    
%\\\hline
%Framing Bias               
%&      \cite{kwak_systematic_2020, hofmann_modeling_2021, mokhberian_moral_2020, Spinde2021f, spinde_exploiting_2022, hamborg_newsalyze_2021} 
%\\\hline
%Political Stance Detection         
%&      \cite{liu_transformer-based_2021, mokhberian_moral_2020, PoliBert20, sinno_political_2022, liu_politics_2022, dinkov_predicting_2019, han_fallacy_2019, baly_we_2020, ruan_pseudo-labelling_2021, lee_neus_2022, chen2020detecting, fan2019a, stefanov_predicting_2020} 
%\\\hline
%Reporting Level Bias       
%&       \cite{tran_how_2020}
%\\\hline
%Spin/Informational Bias    
%&       \cite{van_den_berg_context_2020, fan2019a, chen2020detecting}
%\\\hline
%Gender Bias                
%&       \cite{Mozafari_2020, he_detect_2021}
%\\\hline
%Racial Bias                
%&       \cite{Mozafari_2020, he_detect_2021}
%\\\hline
%Sentiment Analysis         
%&      \cite{Gao_2019, Hamborg_2021}
%\\\hline
%Unreliable / Fake News
%&       \cite{zhou_hidden_2021}
%\end{tabular}
%\caption{Classification of categories of media bias and related concepts investigated using transformer-based approaches.} 
%\label{table:transformers}
%\end{table}

==> Chapters/archive/Methdology_old.tex <==
\section{Methdology} \label{sec:methodology}

We base our literature search strategy largely on the work by Folt\'{y}nek et al. \cite{10.1145/3345317}.
Instead of employing an automated data collection as done by the authors mentioned above, the research papers included in our review have been manually selected via Google Scholar and Mendeley.
Mainly papers from 2018 onwards are considered to cover the rapidly changing research area as precisely as possible. To avoid skipping older groundbreaking or especially relevant work, we also scan relevant primary literature up to 2010.
We consider Google Scholar as an appropriate metadatabase as it complies with the search criteria recommended in systematic literature reviews’ guidelines \cite{Kit04, BRERETON2007571}. 
Google Scholar offers an indexed database of major computer science literature covering ACM Digital Library, ScienceDirect, SpringerLink, and TandFonline, next to grey literature \cite{10.1145/3345317}. 
A large body of literature has found that the coverage offered by Google Scholar does not only meet but exceeds the scope of other search tools “no matter what is identified by target samples, including journals, articles, and citations' '\cite{Fagan_2017}. 
Although previous studies have uncovered nonconformity of commonly used digital libraries in respect to searching facilities as an obstacle for systematic literature reviews in computer science, \cite{BRERETON2007571} this is mitigated by employing Google Scholar.

Fagan et al. \cite{Fagan_2017} view the importance of citations per paper within Google Scholar’s literature rank as too influential. As our study focuses on covering the most impactful media bias papers, this approach of relevance ranking counts as an advantage rather than a drawback. Hence, we use the relevance ranking of Google Scholar and Mendeley. A critical point deemed noteworthy for our paper is the inclusion of predatory journals in Google Scholar’s search results \cite{beall2016best}. Per the guidelines for systematic reviews, which “recommend using additional search tools despite the comprehensive coverage of Google Scholar” \cite{Fagan_2017}, we additionally queried Mendeley. Beyond this, we exclude all papers \cite{aldarmaki-diab-2016-gwu} published by journals found in Beall’s List of Predatory Journals and Publishers\footnote{https://beallslist.weebly.com/standalone-journals.html.}. 
We will outline the different phases of our paper collection procedure in the following. We conducted a review of the first 50 search results from Google Scholar. Next to the paper itself, we considered their references to cover the diversity of aspects media bias research entails. The same procedure was executed for the first 30 search results via Mendeley.
Our procedure is as follows: 

\begin{enumerate}
    \item First, we search for basic papers in the area, independent of the scientific field. Therefore, we use the keywords \textit{media bias} and \textit{slanted coverage} to get an overview. We also try to find literature overviews to identify all related concepts. 
    \item Second, based on the results from the first step, we identify several general concepts that we research in greater detail. We look for: \textit{linguistic media bias, automated detection of media bias, perception of media bias, psychological media bias, social scientific media bias, gender bias, racial bias, hate speech} as well as \textit{automated detection of gender bias / racial bias / hate speech}.  
    \item Third, after reviewing the papers retrieved in the first and second phase, we focus our search on media bias detection and perception in existing text documents. We exclude papers addressing other tasks, such as algorithmic bias and cognitive bias, which are partially also retrieved by our keywords. 
    \item Fourth, we use the exact keywords as we use for Google Scholar with Mendeley to avoid the mentioned selection bias. 
    \item In the fifth phase, we include relevant references of collected papers and papers that publishers’ systems recommended as related to papers in our collection.
\end{enumerate}

By excluding papers that do not report experimental evaluation results, we follow the approach of Folt\'{y}nek et al. \cite{10.1145/3345317}. The chosen papers were first traversed by one author, who extracted their key contents and translated them into a mind map, multi-iteratively reviewed and updated by the other team members. A spreadsheet stored all key features such as tasks, methods, improvements, dataset, results. Table 1 and Table 2 list the numbers of papers retrieved and processed in each data collection phase. 
The measures taken within the collection process have been specifically tailored to bypass common risks faced within literature reviews. Reviews are prone to the incompleteness of data and “deficiencies in the selection, structure, and presentation of the content” \cite{Fagan_2017}, especially when aiming at extensive coverage. We handled this risk by trawling Google Scholar and Mendeley, known to rank very high concerning their scope of academic literature. Additionally, to the deliberate choice of these search engines, we split the process of querying by keywords into multiple steps to achieve fine-grained results. During this process, all single steps were chained to each other by passing on their results to the next step.
We enriched the results derived from our keyword-based search with further papers based on the knowledge of domain experts, i.e., the authors of research papers and literature reviews, and included topic-related suggestions by major publishers, such as Elsevier and ACM.
After our detailed and systematic collection process, we believe in providing a comprehensive review for further state-of-the-art media bias research. The manual exploration of material in different collection stages not only yields a broad but equally deep search that results in the best possible prevention of selection and content subjectivity. Finally, we built on existing reviews while closely following best practice guidelines for systematic reviews.

\subsection{Retrieving and Reviewing Literature on the use of Computer Science Methods for detecting Media Bias}

The core contribution of this paper is a systematic literature review with the goal of describing and structuring the use of computer science methods for detecting media bias. In this section, we describe in detail the procedure of retrieving and reviewing the publications.

\subsubsection{Retrieving Candidate Documents}

\paragraph{Literature databases} 
The main criteria for selecting the literature database for our review are the quality and the completeness of the retrieved candidate documents. 
We chose to retrieve our documents from the dblp computer science bibliography (dblp.org) as well as semantic scholar (https://www.semanticscholar.org/). The dblp (short for DataBase systems and Logic Programming) contains documents from major peer-reviewed computer science journals and proceedings. 
Therefore, literature found on dblp can be considered as solid scientific work. However, publications not found in these sources are not listed in the dblp. Since high-quality publications have not been published in venues or via systems covered by the dblp, we decided to also retrieve literature from semantic scholar, which covers a much larger database. 

\paragraph{Search terms and restrictions}
As search queries for creating the lists of candidates for our literature review, we used the categories and types of bias presented in \ref{sec:framework}. 
We only included literature from 2019 and later in our review to focus on relevant recent publications.

\paragraph{Crawl and results}
A first exploratory evaluation of the results produced by dblp and semantic scholar (now short SeS) already showed a substantial intersection between the results for the different keywords and between the results of both databases. 
Furthermore, the list of results for some of the queries, especially for SeS, was quite large. Therefore, we implemented a crawler to collect, structure, and assemble the search results. 

The dblp crawler was easily implemented since there is an API that allows to filter the results for a certain year range and scientific field (in our case, computer science). 
Searches for the different keywords were carried out separately and then unified, eliminating duplicates. Crawling all potentially relevant literature from dblp resulted in a list of 318 unique publications. 
The SeS crawler had to overcome the hurdle posed by semantic scholar, that API access does not allow for filtering for scientific fields or by year. 
Therefore, some searches resulted in thousands, if not millions, of results. We decided to retrieve the most relevant 1,500 results for each query, then filter for the relevant year range and computer science literature, and finally, remove duplicates from the unified results. 
We ran the crawler for both databases on a single day in May 2022. This produced a list of 1,274 results in total for the SeS crawl. The complete list can be found on Zenodo at [LINK].
As shown in \ref{table:searchResults}, we produced a list of 1209 candidates for the literature review, removing 64 items from the list due to duplication between the SeS and dblp results.  
\begin{center}

\begin{table}[]
\label{table:searchResults}
\caption{Number of publications at each step of literature retrieval and review.} 
\begin{tabular}{l|r}
                   & publications \\ \hline
semantic scholar   & 1,274                   \\
dblp               & 318                    \\\hline 
intersection       & 64                    \\
total, unique      & 1,209                   \\ \hline\hline
after first review & 299                    \\
after final review & 100                   
\end{tabular}
\end{table}
\end{center}


%TR: I'm including an example for the table. Please make them in the same pattern.
\begin{table}[ht!]
    \centering
    \caption{Caption for table.}\label{table:name1}
        \resizebox{0.45\columnwidth}{!}{
            \begin{tabular}{l c c }
            \toprule
             & \multicolumn{2}{c}{Data sources} \\
           \textbf{ Filters} & \textbf{DBLP} & \textbf{Semantic Scholar}\\ 
            \midrule
            Initial        & 318 & 1,274  \\  
            Unique            & 1210 & 254 \\ 
            1\textsuperscript{st} Review & XXX &YYY \\
            2\textsuperscript{nd} Review & ZZZ &WWW \\
            \bottomrule
            \end{tabular}
        }
    
\end{table}




\subsubsection{Literature Review}
\paragraph{How we reviewed the candidates}
All literature was reviewed in multiple steps. First, three reviewers (PhD students in the CS field) briefly examined all candidates to eliminate irrelevant literature. Each piece of literature that seemed to be relevant or that at least was not deemed irrelevant at first glance was then taken into a second and final round of reviews.
In the second review phase, each publication was thoroughly inspected for the use of computer science methods for detecting media bias. If there was the slightest doubt, two other reviewers were consulted, and it was discussed in a group whether the publication was relevant. 

\paragraph{Problems and hurdles in the review process} 
A major problem while labeling for relevance was the high frequency of studies that analyzed bias in texts that have been produced by language models. One could argue that the methods very often could be used to analyze bias in texts produced by humans or that the language model is built with texts produced by humans and therefore reflects biases of humans. However, bias in texts produced by language models essentially is not media bias by our definition of the concept, as described in \ref{sec:bias}. 
Furthermore, We excluded some publications, because we were not able to access them or they were not published in English.







==> Chapters/archive/backup_CS_methods_table.tex <==

%
% really untouched from 22.01.23
\begin{table}[H]
\begin{tabular}{L{2cm}|L{2cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|l}

 & 2019 & 2020 & 2021 & 2022 & total \\\hline
non-artificial neural network machine learning techniques & \cite{ anthonio_team_2019, dinkov_predicting_2019, baly_multi-task_2019, sapiro-gheiler_examining_2019} & \cite{ leavy_uncovering_2020, bourgeois_selection_2018, stefanov_predicting_2020, mokhberian_moral_2020, alzhrani_ideology_2020, kameswari_enhancing_2020, ganguly_empirical_2020, chen_detecting_2020, shahid_detecting_2020, van_den_berg_context_2020} & \cite{ orbach_out_2020, Spinde_2021f, cuellar-hidalgo_luc_2021, zhou_hidden_2021, rao2021gender, Spinde_2021a, bauer_analyzing_2021, krommyda_experimental_2021} &  & 23 \\\hline
non-transformer-based models & \cite{ han_fallacy_2019, Hube_2018b, bordia_identifying_2019, ananya_genderquant_2019, gangula_detecting_2019} & \cite{ baly_we_2020, field_unsupervised_2020, xiao_timme_2020, cruz_document_2020, hube_methods_2020, mathew_hatexplain_2020, Lazaridou_2020, jiang_comparing_2020, webson_undocumented_2020, chen_analyzing_2020} & \cite{ ruan_pseudo-labelling_2021, sinno_political_2022, cuellar-hidalgo_luc_2021, gerald_ki_wei_huang_hyperpartisan_2021, ruan_bias_2021, Spinde_2021a, krommyda_experimental_2021} & \cite{ liu_political_2021, fagni_fine-grained_2022} & 25 \\\hline
traditional NLP techniques & \cite{ wevers_using_2019, badjatiya_stereotypical_2019, sapiro-gheiler_examining_2019, cornelissen_computational_2019} & \cite{ leavy_uncovering_2020, zahid_modeling_2020, niven_measuring_2020, ferrer_discovering_2020, papakyriakopoulos_bias_2020, hamborg_newsalyze_2021, de_arruda_analysing_2020, aires_information_2020, mendelsohn_framework_2020} & \cite{spinde2020a, dalonzo_machine-learning_2021, Spinde2021, kroon_guilty_2021, Kwak_2021, dacon_does_2021, sales_assessing_2021} &  & 20 \\\hline
transformer-based models  & \cite{ han_fallacy_2019, Gao_2019, dinkov_predicting_2019, fan_plain_2019, pryzant_automatically_2019} & \cite{ baly_what_2020, baly_we_2020, li_using_2021, pant_towards_2020, stefanov_predicting_2020, PoliBert20, mokhberian_moral_2020, bhardwaj_investigating_2021, tran_how_2020, mathew_hatexplain_2020, Mozafari_2020, chen_detecting_2020, van_den_berg_context_2020, jiang_comparing_2020, kwak_systematic_2020} & \cite{ huguet_cabot_us_2021, blackledge_transforming_2021, kameswari_towards_2021, madanagopal_towards_2021, ruan_pseudo-labelling_2021, sinno_political_2022, orbach_out_2020, hamborg_newsalyze_2021, Spinde2021f, hofmann_modeling_2021, zhou_hidden_2021, sinha_determining_2021, he_detect_2021, ruan_bias_2021, bauer_analyzing_2021, spinde_interdisciplinary_2021, liu_transformer-based_2021} & \cite{liu_politics_2022, lee_neus_2022, spinde_exploiting_2022, raza_dbias_2022, krieger_2022} & 46 \\\hline
non-artificial neural networks & & & & \cite{ } & ?  \\\hline
graph-based &  & \cite{ stefanov_predicting_2020, chen_neutral_2021, chitra_analyzing_2020} & \cite{ zhou_uncovering_2021, hofmann_modeling_2021, villa_echo_2021, guimaraes_characterizing_2021, dacon_does_2021} & \cite{ guo_modeling_2022} & 8  \\\hline
total & 17 & 41 & 34 & 8 & 
\end{tabular}
\caption{Results of literature study on computer science methods used for media bias detection.} 
\label{table:csmethods1}
\end{table}
